Metal-Poor Stars Observed with the Southern African Large Telescope II. An Extended Sample

We present results from high-resolution (R $\sim 40,000$) spectroscopic observations of over 200 metal-poor stars, mostly selected from the RAVE survey, using the Southern African Large Telescope. We were able to derive stellar parameters for a total of 108 stars; an additional sample of 50 stars from this same effort was previously reported on by Rasmussen et al.. Among our newly reported observations, we identify 84 very metal-poor (VMP; [Fe/H] $< -2.0$, 53 newly identified) stars and 3 extremely metal-poor (EMP; [Fe/H] $< -3.0$, 1 newly identified) stars. The elemental abundances were measured for carbon, as well as several other $\alpha$-elements (Mg, Ca, Sc, Ti), iron-peak elements (Mn, Co, Ni, Zn), and neutron-capture elements (Sr, Ba, Eu). Based on these measurements, the stars are classified by their carbon and neutron-capture abundances into carbon-enhanced metal-poor (CEMP; [C/Fe] $> +0.70$), CEMP sub-classes, and by the level of their $r$-process abundances. A total of 17 are classified as CEMP stars. There are 11 CEMP-$r$ stars (8 newly identified), 1 CEMP-$s$ star (newly identified), 2 possible CEMP-$i$ stars (1 newly identified), and 3 CEMP-no stars (all newly identified) in this work. We found 11 stars (8 newly identified) that are strongly enhanced in $r$-process elements ($r$-II; [Eu/Fe] $> +0.70$), 38 stars (31 newly identified) that are moderately enhanced in $r$-process elements ($r$-I; $+0.30 < $ [Eu/Fe] $\leq +0.70$), and 1 newly identified limited-$r$ star.

==> Table2_DateandRV.tex <==
\begin{deluxetable*}{ccccc}[t]
\tablecaption{\label{tab:rv} Position, Date of Observation, and Radial Velocity}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Name}  &
\colhead{RA} &
\colhead{Dec} &
\colhead{UT Date} &
\colhead{RV} 
\\
& \colhead{(degrees)} & \colhead{(degrees)} &  & \colhead{(km s$^{-1}$)}
}
\startdata
RAVE J000438.4-540134 & 	 +1.1583 & 	 $-$54.0261 & 	October 1 2018 & 	 +191.2$\pm$2.1 \\
RAVE J001236.5-181631 & 	 +3.1500 & 	 $-$18.2750 & 	July 4 2017 & 	 $-$121.8$\pm$1.3 \\
RAVE J003946.9-684957 & 	 +9.9458 & 	 $-$68.8331 & 	November 28 2018 & 	 +81.3$\pm$1.2 \\
RAVE J010839.6-285701 & 	 +17.1667 & 	 $-$28.9500 & 	July 7 2017 & 	 +124.6$\pm$3.6 \\
2MASS J01162885-5343408 & 	 +19.1208 & 	 $-$53.7281 & 	July 29 2018 & 	 $-$16.7$\pm$0.8 \\
2MASS J01201051-4849461 & 	 +20.0458 & 	 $-$48.8300 & 	October 21 2018 & 	 $-$64.1$\pm$7.9 \\
RAVE J012931.1-160046 & 	 +22.3792 & 	 $-$16.0131 & 	June 12 2017 & 	 +111.1$\pm$9.3 \\
RAVE J013807.0-195210 & 	 +24.5292 & 	 $-$19.8689 & 	October 21 2018 & 	 $-$66.1$\pm$3.1 \\
RAVE J014254.2-503249 & 	 +25.7250 & 	 $-$50.5469 & 	June 21 2017 & 	 +143.9$\pm$1.7 \\
RAVE J014908.0-491143 & 	 +27.2833 & 	 $-$49.1950 & 	June 13 2017 & 	 +72.6$\pm$2.8 \\
RAVE J021110.2-191124 & 	 +32.7917 & 	 $-$19.1900 & 	October 4 2017 & 	 $-$92.8$\pm$0.4 \\
RAVE J022013.3-601436 & 	 +35.0542 & 	 $-$60.2431 & 	September 27 2018 & 	 +197.0$\pm$3.4 \\
RAVE J030639.1-692040 & 	 +46.6625 & 	 $-$69.3439 & 	October 30 2018 & 	 +205.8$\pm$4.6 \\
2MASS J03135637-6554095 & 	 +48.4833 & 	 $-$65.9031 & 	September 22 2018 & 	 +163.3$\pm$3.7 \\
RAVE J034228.2-650036 & 	 +55.6167 & 	 $-$65.0100 & 	August 24 2018 & 	 +103.0$\pm$3.5 \\
2MASS J04042657-2229357 & 	 +61.1125 & 	 $-$22.4931 & 	October 21 2018 & 	 $-$37.3$\pm$2.5 \\
RAVE J040658.7-540556 & 	 +61.7458 & 	 $-$54.0989 & 	October 27 2018 & 	 +91.4$\pm$4.8 \\
RAVE J045322.6-221040 & 	 +73.3458 & 	 $-$22.1781 & 	October 27 2017 & 	 +1.4$\pm$1.5 \\
2MASS J05023178-4540502 & 	 +75.6333 & 	 $-$45.6811 & 	October 26 2018 & 	 +115.5$\pm$4.0 \\
RAVE J050600.7-351056 & 	 +76.5042 & 	 $-$35.1819 & 	October 21 2018 & 	 +146.1$\pm$3.5 \\
RAVE J050947.6-442317 & 	 +77.4500 & 	 $-$44.3881 & 	August 24 2018 & 	 $-$58.9$\pm$3.5 \\
RAVE J053817.0-751621 & 	 +84.5708 & 	 $-$75.2719 & 	November 6 2017 & 	 +61.7$\pm$2.0 \\
2MASS J05510847-5523127 & 	 +87.7833 & 	 $-$55.3869 & 	October 23 2018 & 	 +292.8$\pm$4.8 \\
RAVE J061950.0-531212 & 	 +94.9583 & 	 $-$53.2031 & 	October 27 2017 & 	 +126.5$\pm$2.0 \\
2MASS J06340181-4707492 & 	 +98.5083 & 	 $-$47.1300 & 	October 27 2018 & 	 +314.1$\pm$3.7 \\
RAVE J063736.3-692947 & 	 +99.4000 & 	 $-$69.4961 & 	December 10 2017 & 	 +178.4$\pm$3.5 \\
RAVE J070520.3-334324 & 	 +106.3333 & 	 $-$33.7231 & 	October 5 2017 & 	 +393.2$\pm$5.5 \\
RAVE J074824.3-483141 & 	 +117.1000 & 	 $-$48.5281 & 	April 22 2017 & 	 +337.1$\pm$0.2 \\
RAVE J100709.2-180947 & 	 +151.7875 & 	 $-$18.1631 & 	December 6 2017 & 	 +241.8$\pm$2.7 \\
RAVE J100824.9-231412 & 	 +152.1042 & 	 $-$23.2369 & 	June 11 2017 & 	 +161.0$\pm$0.1 \\
RAVE J101621.6-295952 & 	 +154.0917 & 	 $-$29.9981 & 	June 1 2017 & 	 +452.0$\pm$0.0 \\
RAVE J112651.4-180530 & 	 +171.7125 & 	 $-$18.0919 & 	March 26 2019 & 	 +58.6$\pm$0.6 \\
RAVE J113508.3-111328 & 	 +173.7833 & 	 $-$11.2239 & 	April 15 2017 & 	 +129.1$\pm$0.4 \\
RAVE J114444.8-112817 & 	 +176.1875 & 	 $-$11.4711 & 	April 11 2017 & 	 +177.8$\pm$3.4 \\
RAVE J115337.3-020037 & 	 +178.4042 & 	 $-$2.0100 & 	March 26 2019 & 	 $-$31.5$\pm$1.1 \\
RAVE J115941.7-382043 & 	 +179.9250 & 	 $-$38.3450 & 	April 17 2017 & 	 +51.7$\pm$3.8 \\
RAVE J123550.1-313111 & 	 +188.9583 & 	 $-$31.5200 & 	April 18 2017 & 	 +216.6$\pm$6.5 \\
RAVE J115941.7-382043 & 	 +190.4792 & 	 $-$8.9500 & 	February 8 2018 & 	 +21.4$\pm$2.5 \\
RAVE J124718.3-555047 & 	 +191.8250 & 	 $-$55.8461 & 	January 28 2018 & 	 +147.7$\pm$2.7 \\
RAVE J124753.3-390802 & 	 +191.9708 & 	 $-$39.1339 & 	January 15 2018 & 	 +1.2$\pm$0.3 \\
RAVE J125728.3-512522 & 	 +194.3667 & 	 $-$51.4231 & 	July 8 2017 & 	 +62.1$\pm$1.7 \\
RAVE J125807.3-450627 & 	 +194.5292 & 	 $-$45.1081 & 	June 5 2017 & 	 +324.9$\pm$8.6 \\
RAVE J130231.2-144805 & 	 +195.6292 & 	 $-$14.8011 & 	July 7 2017 & 	 +185.4$\pm$4.0 \\
RAVE J130404.1-240837 & 	 +196.0167 & 	 +13.0678 & 	June 2 2017 & 	 +137.4$\pm$2.2 \\
RAVE J130455.0-371249 & 	 +196.2292 & 	 $-$37.2139 & 	March 26 2019 & 	 $-$82.2$\pm$12.4 \\
RAVE J133352.8-262354 & 	 +203.4708 & 	 $-$26.3981 & 	July 6 2017 & 	 +92.7$\pm$1.3 \\
RAVE J134723.7-314409 & 	 +206.8500 & 	 $-$31.7361 & 	June 14 2017 & 	 +74.5$\pm$2.5 \\
RAVE J135735.4-303249 & 	 +209.4000 & 	 $-$30.5469 & 	June 1 2017 & 	 $-$8.5$\pm$3.2 \\
RAVE J140329.0-525043 & 	 +210.8708 & 	 $-$52.8450 & 	March 26 2019 & 	 +66.4$\pm$4.9 \\
RAVE J140335.4-333526 & 	 +210.9000 & 	 $-$33.5900 & 	March 26 2019 & 	 +210.4$\pm$5.6 \\
RAVE J141126.2-113746 & 	 +212.8583 & 	 $-$11.6289 & 	January 29 2019 & 	 +26.3$\pm$4.4 \\
RAVE J141253.2-355256 & 	 +213.2208 & 	 $-$35.8819 & 	July 11 2017 & 	 +354.0$\pm$5.3 \\
RAVE J153830.9-180424 & 	 +234.6292 & 	 $-$18.0731 & 	May 13 2017 & 	 +132.1$\pm$3.4 \\
RAVE J155211.1-143037 & 	 +238.0458 & 	 $-$14.5100 & 	June 1 2017 & 	 $-$53.9$\pm$2.2 \\
RAVE J155829.6-122434 & 	 +239.6250 & 	 $-$12.4100 & 	April 18 2017 & 	 +68.2$\pm$0.4 \\
RAVE J160245.0-152102 & 	 +240.6875 & 	 $-$15.3500 & 	April 19 2017 & 	 +82.6$\pm$4.9 \\
RAVE J161847.0-014540 & 	 +244.6958 & 	 $-$1.7611 & 	June 5 2017 & 	 $-$300.2$\pm$1.7 \\
RAVE J161943.1-022431 & 	 +244.9292 & 	 $-$2.4081 & 	June 5 2017 & 	 $-$221.2$\pm$4.0 \\
RAVE J165300.5-005507 & 	 +253.2500 & 	 $-$0.9189 & 	May 18 2017 & 	 $-$36.0$\pm$3.0 \\
2MASS J17163340-7009028 & 	 +259.1375 & 	 $-$70.1511 & 	June 8 2018 & 	 $-$28.3$\pm$1.2 \\
RAVE J175159.8-475131 & 	 +268.0000 & 	 $-$47.8589 & 	February 23 2019 & 	 +1.0$\pm$3.6 \\
RAVE J180242.3-440443 & 	 +270.6750 & 	 $-$44.0781 & 	June 13 2018 & 	 $-$225.7$\pm$5.1 \\
RAVE J183108.2-491105 & 	 +277.7833 & 	 $-$49.1850 & 	July 23 2018 & 	 $-$164.6$\pm$1.6 \\
RAVE J183623.2-642812 & 	 +279.0958 & 	 $-$64.4700 & 	March 23 2019 & 	 $-$41.5$\pm$5.7 \\
2MASS J19031845-5138510 & 	 +285.8250 & 	 $-$51.6481 & 	October 17 2018 & 	 +185.8$\pm$5.2 \\
RAVE J190733.1-415832 & 	 +286.8875 & 	 $-$41.9750 & 	June 16 2017 & 	 +173.0$\pm$1.1 \\
RAVE J190923.1-435357 & 	 +287.3458 & 	 $-$43.8989 & 	June 16 2017 & 	 +18.0$\pm$1.9 \\
RAVE J191755.9-544015 & 	 +289.4833 & 	 $-$54.6711 & 	April 19 2017 & 	 +6.0$\pm$1.4 \\
RAVE J192325.2-583341 & 	 +290.8542 & 	 $-$58.5611 & 	September 3 2018 & 	 +143.8$\pm$7.0 \\
RAVE J192819.9-633935 & 	 +292.0833 & 	 $-$63.6600 & 	May 19 2017 & 	 $-$122.8$\pm$2.4 \\
RAVE J193102.8-440158 & 	 +292.7625 & 	 $-$44.0331 & 	June 15 2017 & 	 $-$72.8$\pm$4.4 \\
RAVE J194318.7-594820 & 	 +295.8292 & 	 $-$59.8061 & 	September 29 2018 & 	 +23.2$\pm$6.1 \\
RAVE J194319.0-405425 & 	 +295.8292 & 	 $-$40.9069 & 	July 4 2017 & 	 $-$95.3$\pm$0.6 \\
RAVE J194550.6-392631 & 	 +296.4625 & 	 $-$39.4419 & 	May 6 2017 & 	 $-$39.0$\pm$1.3 \\
RAVE J200034.7-342004 & 	 +300.1458 & 	 $-$34.3350 & 	July 1 2017 & 	 $-$17.0$\pm$1.4 \\
RAVE J200057.7-254149 & 	 +300.2417 & 	 $-$25.6969 & 	June 18 2017 & 	 +134.6$\pm$2.4 \\
RAVE J201007.1-515502 & 	 +302.5292 & 	 $-$51.9169 & 	July 14 2017 & 	 +166.1$\pm$0.2 \\
RAVE J202029.2-270735 & 	 +305.1208 & 	 $-$27.1261 & 	June 16 2017 & 	 $-$39.0$\pm$1.1 \\
RAVE J202432.1-151029 & 	 +306.1333 & 	 $-$15.1750 & 	June 25 2017 & 	 $-$41.0$\pm$1.9 \\
RAVE J202434.5-423334 & 	 +306.1458 & 	 $-$42.5589 & 	October 7 2017 & 	 +259.9$\pm$0.1 \\
2MASS J20264253-1656467 & 	 +306.6750 & 	 $-$16.9461 & 	July 5 2018 & 	 $-$58.2$\pm$2.6 \\
RAVE J202654.7-595013 & 	 +306.7292 & 	 $-$59.8369 & 	September 21 2018 & 	 +138.6$\pm$1.5 \\
RAVE J203428.4-241830 & 	 +308.6167 & 	 $-$24.3081 & 	October 5 2017 & 	 +78.6$\pm$2.4 \\
RAVE J203622.6-071420 & 	 +309.0958 & 	 $-$7.2389 & 	July 6 2018 & 	 $-$320.7$\pm$1.2 \\
RAVE J203706.4-122125 & 	 +309.2750 & 	 $-$12.3569 & 	July 19 2018 & 	 $-$28.7$\pm$1.9 \\
RAVE J204355.8-563629 & 	 +310.9833 & 	 $-$56.6081 & 	July 28 2018 & 	 +190.3$\pm$0.6 \\
RAVE J204450.7-371400 & 	 +311.2125 & 	 $-$37.2331 & 	April 17 2019 & 	 +97.2$\pm$4.1 \\
RAVE J204954.4-480045 & 	 +312.4750 & 	 $-$48.0131 & 	October 28 2017 & 	 +103.9$\pm$2.0 \\
RAVE J205149.7-615801 & 	 +312.9583 & 	 $-$61.9669 & 	May 17 2017 & 	 $-$107.0$\pm$6.8 \\
RAVE J205609.1-133118 & 	 +314.0375 & 	 $-$13.5219 & 	May 7 2017 & 	 +93.7$\pm$2.8 \\
RAVE J210634.7-495750 & 	 +316.6458 & 	 $-$49.9639 & 	July 21 2018 & 	 $-$43.3$\pm$4.1 \\
RAVE J210642.9-682827 & 	 +316.6792 & 	 $-$68.4739 & 	May 31 2017 & 	 $-$85.3$\pm$5.0 \\
RAVE J211525.5-150331 & 	 +318.8542 & 	 $-$15.0589 & 	July 21 2018 & 	 $-$16.0$\pm$2.1 \\
RAVE J211927.1-402908 & 	 +319.8625 & 	 $-$40.4861 & 	October 5 2017 & 	 +116.9$\pm$3.5 \\
RAVE J212921.0-620915 & 	 +322.3375 & 	 $-$62.1539 & 	July 25 2018 & 	 $-$18.0$\pm$1.6 \\
RAVE J215118.3-135937 & 	 +327.8250 & 	 $-$13.9939 & 	November 6 2017 & 	 $-$67.3$\pm$2.1 \\
RAVE J220211.8-441702 & 	 +330.5500 & 	 $-$44.2839 & 	October 29 2017 & 	 +151.6$\pm$2.7 \\
RAVE J220403.6-402919 & 	 +331.0167 & 	 $-$40.4889 & 	July 23 2018 & 	 $-$44.8$\pm$1.5 \\
2MASS J22122728-6810067 & 	 +333.1125 & 	 $-$68.1689 & 	September 21 2018 & 	 +4.8$\pm$4.5 \\
RAVE J222236.0-013827 & 	 +335.6500 & 	 $-$1.6411 & 	July 8 2018 & 	 $-$88.4$\pm$2.0 \\
RAVE J223716.2-160801 & 	 +339.3167 & 	 $-$16.1339 & 	October 27 2017 & 	 +25.1$\pm$6.2 \\
RAVE J224927.6-223829 & 	 +342.3667 & 	 $-$22.6411 & 	July 6 2017 & 	 $-$20.9$\pm$1.4 \\
RAVE J225319.9-224856 & 	 +343.3333 & 	 $-$22.8150 & 	October 7 2017 & 	 +16.4$\pm$1.7 \\
RAVE J225926.9-523733 & 	 +344.8625 & 	 $-$52.6261 & 	May 31 2017 & 	 +105.7$\pm$5.1 \\
RAVE J230222.9-683323 & 	 +345.5958 & 	 $-$68.5561 & 	July 29 2018 & 	 +139.8$\pm$2.2 \\
RAVE J231300.0-450707 & 	 +348.2500 & 	 $-$45.1181 & 	June 16 2017 & 	 $-$113.4$\pm$3.5 \\
2MASS J23131638-7011223 & 	 +348.3167 & 	 $-$70.1900 & 	July 30 2018 & 	 +232.7$\pm$2.5 \\
\enddata
\tablecomments{This table is a stub; the full table is available in the electronic edition.}
\end{deluxetable*}

==> Table3_SNandStellarParam.tex <==
\startlongtable

\begin{deluxetable*}{ccccccc}
\tablecaption{\label{tab:sp_full}Signal-to-Noise and Stellar Parameters}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Name}  &
\colhead{Other Name} &
\colhead{S/N } & 
\colhead{$T_{\rm eff}$} &
\colhead{log $g$} &
\colhead{$\xi$} &
\colhead{[Fe/H]}\\
& & \colhead{(5033\,\AA)}&\colhead{(K)} & \colhead{(cgs)} & \colhead{(km s$^{-1}$)} & \colhead{} 
}
\startdata
RAVE J000438.4-540134 & 	--- & 	30 & 	4678$\pm$150 & 	1.51$\pm$0.30 & 	1.87$\pm$0.20 & 	$-$2.38$\pm$0.10 \\
RAVE J001236.5-181631 & 	--- & 	57 & 	5073$\pm$150 & 	2.41$\pm$0.30 & 	1.63$\pm$0.20 & 	$-$2.41$\pm$0.09 \\
RAVE J003946.9-684957 & 	--- & 	32 & 	4631$\pm$150 & 	1.16$\pm$0.30 & 	1.88$\pm$0.20 & 	$-$2.62$\pm$0.10 \\
RAVE J010839.6-285701 & 	SMSS J010839.58-285701.5 & 	27 & 	4843$\pm$150 & 	1.17$\pm$0.30 & 	1.61$\pm$0.20 & 	$-$2.87$\pm$0.14 \\
2MASS J01162885-5343408 & 	--- & 	32 & 	4808$\pm$150 & 	1.54$\pm$0.30 & 	2.09$\pm$0.20 & 	$-$2.76$\pm$0.14 \\
2MASS J01201051-4849461 & 	--- & 	31 & 	4797$\pm$150 & 	1.69$\pm$0.30 & 	1.08$\pm$0.20 & 	$-$2.17$\pm$0.14 \\
RAVE J012931.1-160046 & 	BPS CS 31082-0001, BD-16 251 & 	49 & 	4676$\pm$150 & 	1.01$\pm$0.30 & 	2.23$\pm$0.20 & 	$-$2.98$\pm$0.15 \\
RAVE J013807.0-195210 & 	--- & 	34 & 	4898$\pm$150 & 	2.48$\pm$0.30 & 	1.28$\pm$0.20 & 	$-$2.05$\pm$0.14 \\
RAVE J014254.2-503249 & 	--- & 	37 & 	5109$\pm$150 & 	2.69$\pm$0.30 & 	1.45$\pm$0.20 & 	$-$2.18$\pm$0.11 \\
RAVE J014908.0-491143 & 	HE 0147-4926, CD-49 506 & 	66 & 	4556$\pm$150 & 	0.72$\pm$0.30 & 	2.14$\pm$0.20 & 	$-$3.08$\pm$0.10 \\
RAVE J021110.2-191124 & 	--- & 	39 & 	5098$\pm$150 & 	2.59$\pm$0.30 & 	1.47$\pm$0.20 & 	$-$2.37$\pm$0.10 \\
RAVE J022013.3-601436 & 	--- & 	34 & 	4818$\pm$150 & 	1.75$\pm$0.30 & 	1.57$\pm$0.20 & 	$-$1.67$\pm$0.14 \\
RAVE J030639.1-692040 & 	--- & 	36 & 	4644$\pm$150 & 	1.04$\pm$0.30 & 	1.62$\pm$0.20 & 	$-$2.79$\pm$0.13 \\
2MASS J03135637-6554095 & 	--- & 	32 & 	4867$\pm$150 & 	1.82$\pm$0.30 & 	1.79$\pm$0.20 & 	$-$2.43$\pm$0.14 \\
RAVE J034228.2-650036 & 	CPD -65 261 & 	54 & 	4768$\pm$150 & 	1.66$\pm$0.30 & 	1.64$\pm$0.20 & 	$-$2.30$\pm$0.10 \\
2MASS J04042657-2229357 & 	--- & 	22 & 	4996$\pm$150 & 	2.69$\pm$0.30 & 	1.64$\pm$0.20 & 	$-$1.86$\pm$0.16 \\
RAVE J040658.7-540556 & 	--- & 	37 & 	5104$\pm$150 & 	2.23$\pm$0.30 & 	1.79$\pm$0.20 & 	$-$2.49$\pm$0.12 \\
RAVE J045322.6-221040 & 	--- & 	51 & 	6281$\pm$150 & 	4.09$\pm$0.30 & 	1.61$\pm$0.20 & 	$-$2.31$\pm$0.10 \\
2MASS J05023178-4540502 & 	--- & 	27 & 	5157$\pm$150 & 	4.03$\pm$0.30 & 	1.21$\pm$0.20 & 	$-$0.76$\pm$0.17 \\
RAVE J050600.7-351056 & 	--- & 	34 & 	5236$\pm$150 & 	3.24$\pm$0.30 & 	1.71$\pm$0.20 & 	$-$1.98$\pm$0.14 \\
RAVE J050947.6-442317 & 	HE 0508-4426, CD-44 1896, HD 273482 & 	46 & 	5535$\pm$150 & 	3.34$\pm$0.30 & 	1.47$\pm$0.20 & 	$-$2.50$\pm$0.10 \\
RAVE J053817.0-751621 & 	--- & 	49 & 	4716$\pm$150 & 	1.33$\pm$0.30 & 	1.18$\pm$0.20 & 	$-$2.03$\pm$0.14 \\
2MASS J05510847-5523127 & 	--- & 	41 & 	4851$\pm$150 & 	1.72$\pm$0.30 & 	1.40$\pm$0.20 & 	$-$2.31$\pm$0.10 \\
RAVE J061950.0-531212 & 	--- & 	40 & 	5223$\pm$150 & 	2.96$\pm$0.30 & 	1.78$\pm$0.20 & 	$-$2.09$\pm$0.16 \\
2MASS J06340181-4707492 & 	--- & 	50 & 	4769$\pm$150 & 	1.98$\pm$0.30 & 	1.17$\pm$0.20 & 	$-$2.26$\pm$0.10 \\
RAVE J063736.3-692947 & 	--- & 	25 & 	5773$\pm$150 & 	3.43$\pm$0.30 & 	1.28$\pm$0.20 & 	$-$1.67$\pm$0.24 \\
RAVE J070520.3-334324 & 	--- & 	44 & 	4755$\pm$150 & 	1.36$\pm$0.30 & 	1.93$\pm$0.20 & 	$-$2.43$\pm$0.13 \\
RAVE J074824.3-483141 & 	--- & 	84 & 	5465$\pm$150 & 	1.88$\pm$0.30 & 	2.29$\pm$0.20 & 	$-$2.01$\pm$0.11 \\
RAVE J100709.2-180947 & 	--- & 	25 & 	4681$\pm$150 & 	1.51$\pm$0.30 & 	1.47$\pm$0.20 & 	$-$1.92$\pm$0.15 \\
RAVE J100824.9-231412 & 	--- & 	22 & 	4719$\pm$150 & 	1.18$\pm$0.30 & 	1.87$\pm$0.20 & 	$-$1.95$\pm$0.13 \\
RAVE J101621.6-295952 & 	--- & 	66 & 	4866$\pm$150 & 	2.00$\pm$0.30 & 	1.80$\pm$0.20 & 	$-$2.12$\pm$0.12 \\
RAVE J112651.4-180530 & 	--- & 	30 & 	5045$\pm$150 & 	2.26$\pm$0.30 & 	1.81$\pm$0.20 & 	$-$2.52$\pm$0.13 \\
RAVE J113508.3-111328 & 	--- & 	39 & 	5980$\pm$150 & 	4.08$\pm$0.30 & 	1.44$\pm$0.20 & 	$-$1.32$\pm$0.12 \\
RAVE J114444.8-112817 & 	BD-10 3332 & 	70 & 	4988$\pm$150 & 	2.41$\pm$0.30 & 	1.34$\pm$0.20 & 	$-$2.63$\pm$0.08 \\
RAVE J115337.3-020037 & 	BD-01 2582 & 	43 & 	5151$\pm$150 & 	2.74$\pm$0.30 & 	1.88$\pm$0.20 & 	$-$2.43$\pm$0.12 \\
RAVE J115941.7-382043 & 	--- & 	52 & 	4915$\pm$150 & 	2.63$\pm$0.30 & 	0.99$\pm$0.20 & 	$-$1.23$\pm$0.10 \\
RAVE J123550.1-313111 & 	HE 1233-3114, CD-30 10002 & 	27 & 	4706$\pm$150 & 	1.32$\pm$0.30 & 	2.31$\pm$0.20 & 	$-$2.59$\pm$0.13 \\
RAVE J115941.7-382043 & 	--- & 	31 & 	5926$\pm$150 & 	3.56$\pm$0.30 & 	1.66$\pm$0.20 & 	$-$2.27$\pm$0.16 \\
RAVE J124718.3-555047 & 	--- & 	29 & 	4815$\pm$150 & 	1.79$\pm$0.30 & 	1.87$\pm$0.20 & 	$-$2.00$\pm$0.13 \\
RAVE J124753.3-390802 & 	--- & 	29 & 	4427$\pm$150 & 	0.78$\pm$0.30 & 	2.71$\pm$0.20 & 	$-$2.17$\pm$0.11 \\
RAVE J125728.3-512522 & 	--- & 	50 & 	4638$\pm$150 & 	1.28$\pm$0.30 & 	2.08$\pm$0.20 & 	$-$2.47$\pm$0.11 \\
RAVE J125807.3-450627 & 	--- & 	42 & 	4446$\pm$150 & 	1.22$\pm$0.30 & 	2.75$\pm$0.20 & 	$-$2.07$\pm$0.16 \\
RAVE J130231.2-144805 & 	--- & 	57 & 	5797$\pm$150 & 	3.58$\pm$0.30 & 	1.31$\pm$0.20 & 	$-$1.75$\pm$0.08 \\
RAVE J130404.1-240837 & 	--- & 	63 & 	4943$\pm$150 & 	2.24$\pm$0.30 & 	2.08$\pm$0.20 & 	$-$2.17$\pm$0.12 \\
RAVE J130455.0-371249 & 	--- & 	43 & 	6279$\pm$150 & 	3.87$\pm$0.30 & 	1.78$\pm$0.20 & 	$-$0.89$\pm$0.08 \\
RAVE J133352.8-262354 & 	--- & 	54 & 	4768$\pm$150 & 	1.54$\pm$0.30 & 	1.56$\pm$0.20 & 	$-$2.27$\pm$0.09 \\
RAVE J134723.7-314409 & 	CD-31 10642 & 	61 & 	4988$\pm$150 & 	2.37$\pm$0.30 & 	1.54$\pm$0.20 & 	$-$1.99$\pm$0.11 \\
RAVE J135735.4-303249 & 	--- & 	49 & 	4968$\pm$150 & 	2.19$\pm$0.30 & 	1.52$\pm$0.20 & 	$-$2.46$\pm$0.10 \\
RAVE J140329.0-525043 & 	--- & 	38 & 	5075$\pm$150 & 	2.72$\pm$0.30 & 	1.22$\pm$0.20 & 	$-$1.93$\pm$0.10 \\
RAVE J140335.4-333526 & 	CD-33 9514 & 	27 & 	4876$\pm$150 & 	1.76$\pm$0.30 & 	1.91$\pm$0.20 & 	$-$2.75$\pm$0.10 \\
RAVE J141126.2-113746 & 	--- & 	52 & 	4484$\pm$150 & 	1.00$\pm$0.30 & 	3.80$\pm$0.20 & 	$-$2.75$\pm$0.12 \\
RAVE J141253.2-355256 & 	--- & 	31 & 	4719$\pm$150 & 	1.47$\pm$0.30 & 	1.38$\pm$0.20 & 	$-$2.45$\pm$0.08 \\
RAVE J153830.9-180424 & 	--- & 	58 & 	4704$\pm$150 & 	1.47$\pm$0.30 & 	1.42$\pm$0.20 & 	$-$2.20$\pm$0.11 \\
RAVE J155211.1-143037 & 	G 152-58 & 	49 & 	5918$\pm$150 & 	4.22$\pm$0.30 & 	1.16$\pm$0.20 & 	$-$1.60$\pm$0.12 \\
RAVE J155829.6-122434 & 	--- & 	63 & 	4837$\pm$150 & 	1.00$\pm$0.30 & 	2.21$\pm$0.20 & 	$-$2.82$\pm$0.09 \\
RAVE J160245.0-152102 & 	BD-14 4336 & 	81 & 	5026$\pm$150 & 	2.62$\pm$0.30 & 	1.25$\pm$0.20 & 	$-$2.05$\pm$0.10 \\
RAVE J161847.0-014540 & 	--- & 	47 & 	4748$\pm$150 & 	1.61$\pm$0.30 & 	1.69$\pm$0.20 & 	$-$2.09$\pm$0.10 \\
RAVE J161943.1-022431 & 	--- & 	48 & 	4958$\pm$150 & 	2.29$\pm$0.30 & 	1.58$\pm$0.20 & 	$-$2.24$\pm$0.09 \\
RAVE J165300.5-005507 & 	--- & 	55 & 	4532$\pm$150 & 	0.89$\pm$0.30 & 	1.95$\pm$0.20 & 	$-$1.63$\pm$0.13 \\
2MASS J17163340-7009028 & 	--- & 	32 & 	4556$\pm$150 & 	1.02$\pm$0.30 & 	2.67$\pm$0.20 & 	$-$2.69$\pm$0.15 \\
RAVE J175159.8-475131 & 	--- & 	66 & 	4428$\pm$150 & 	1.42$\pm$0.30 & 	2.55$\pm$0.20 & 	$-$2.20$\pm$0.11 \\
RAVE J180242.3-440443 & 	--- & 	28 & 	4449$\pm$150 & 	0.69$\pm$0.30 & 	1.78$\pm$0.20 & 	$-$1.88$\pm$0.12 \\
RAVE J183108.2-491105 & 	--- & 	45 & 	4420$\pm$150 & 	0.69$\pm$0.30 & 	2.28$\pm$0.20 & 	$-$2.08$\pm$0.18 \\
RAVE J183623.2-642812 & 	--- & 	28 & 	4902$\pm$150 & 	1.79$\pm$0.30 & 	1.83$\pm$0.20 & 	$-$2.54$\pm$0.08 \\
2MASS J19031845-5138510 & 	--- & 	26 & 	4971$\pm$150 & 	2.33$\pm$0.30 & 	2.01$\pm$0.20 & 	$-$2.15$\pm$0.16 \\
RAVE J190733.1-415832 & 	--- & 	30 & 	4429$\pm$150 & 	0.60$\pm$0.30 & 	2.40$\pm$0.20 & 	$-$2.44$\pm$0.13 \\
RAVE J190923.1-435357 & 	--- & 	39 & 	4635$\pm$150 & 	0.93$\pm$0.30 & 	2.04$\pm$0.20 & 	$-$2.05$\pm$0.14 \\
RAVE J191755.9-544015 & 	CD-54 8237 & 	75 & 	4635$\pm$150 & 	1.09$\pm$0.30 & 	1.90$\pm$0.20 & 	$-$2.81$\pm$0.10 \\
RAVE J192325.2-583341 & 	--- & 	48 & 	4829$\pm$150 & 	1.80$\pm$0.30 & 	1.83$\pm$0.20 & 	$-$2.41$\pm$0.13 \\
RAVE J192819.9-633935 & 	--- & 	55 & 	4789$\pm$150 & 	1.57$\pm$0.30 & 	1.79$\pm$0.20 & 	$-$2.40$\pm$0.11 \\
RAVE J193102.8-440158 & 	--- & 	58 & 	4562$\pm$150 & 	1.07$\pm$0.30 & 	1.77$\pm$0.20 & 	$-$2.28$\pm$0.13 \\
RAVE J194319.0-405425 & 	--- & 	62 & 	5889$\pm$150 & 	3.40$\pm$0.30 & 	1.59$\pm$0.20 & 	$-$1.72$\pm$0.10 \\
RAVE J194318.7-594820 & 	--- & 	28 & 	5115$\pm$150 & 	2.59$\pm$0.30 & 	1.73$\pm$0.20 & 	$-$2.17$\pm$0.13 \\
RAVE J194550.6-392631 & 	--- & 	66 & 	4682$\pm$150 & 	1.28$\pm$0.30 & 	1.96$\pm$0.20 & 	$-$2.97$\pm$0.09 \\
RAVE J200034.7-342004 & 	--- & 	29 & 	5138$\pm$150 & 	2.86$\pm$0.30 & 	1.66$\pm$0.20 & 	$-$2.12$\pm$0.14 \\
RAVE J200057.7-254149 & 	--- & 	69 & 	4654$\pm$150 & 	1.23$\pm$0.30 & 	1.90$\pm$0.20 & 	$-$2.09$\pm$0.11 \\
RAVE J201007.1-515502 & 	--- & 	60 & 	4534$\pm$150 & 	0.83$\pm$0.30 & 	2.11$\pm$0.20 & 	$-$2.56$\pm$0.12 \\
RAVE J202029.2-270735 & 	--- & 	32 & 	4625$\pm$150 & 	0.95$\pm$0.30 & 	2.55$\pm$0.20 & 	$-$3.01$\pm$0.11 \\
RAVE J202432.1-151029 & 	BD-15 5652 & 	60 & 	4728$\pm$150 & 	1.79$\pm$0.30 & 	1.61$\pm$0.20 & 	$-$1.71$\pm$0.12 \\
RAVE J202434.5-423334 & 	--- & 	28 & 	5024$\pm$150 & 	2.13$\pm$0.30 & 	1.47$\pm$0.20 & 	$-$2.68$\pm$0.17 \\
2MASS J20264253-1656467 & 	--- & 	44 & 	4479$\pm$150 & 	0.95$\pm$0.30 & 	1.91$\pm$0.20 & 	$-$1.97$\pm$0.16 \\
RAVE J202654.7-595013 & 	--- & 	61 & 	4881$\pm$150 & 	2.21$\pm$0.30 & 	1.11$\pm$0.20 & 	$-$2.05$\pm$0.11 \\
RAVE J203428.4-241830 & 	--- & 	51 & 	4671$\pm$150 & 	1.27$\pm$0.30 & 	1.44$\pm$0.20 & 	$-$2.48$\pm$0.12 \\
RAVE J203622.6-071420 & 	--- & 	81 & 	4427$\pm$150 & 	0.83$\pm$0.30 & 	3.75$\pm$0.20 & 	$-$2.59$\pm$0.11 \\
RAVE J203706.4-122125 & 	--- & 	52 & 	4451$\pm$150 & 	0.83$\pm$0.30 & 	2.84$\pm$0.20 & 	$-$2.61$\pm$0.14 \\
RAVE J204355.8-563629 & 	--- & 	59 & 	4880$\pm$150 & 	2.15$\pm$0.30 & 	1.19$\pm$0.20 & 	$-$2.07$\pm$0.11 \\
RAVE J204450.7-371400 & 	--- & 	41 & 	4710$\pm$150 & 	1.62$\pm$0.30 & 	2.75$\pm$0.20 & 	$-$2.72$\pm$0.11 \\
RAVE J204954.4-480045 & 	--- & 	72 & 	5125$\pm$150 & 	2.67$\pm$0.30 & 	1.55$\pm$0.20 & 	$-$1.82$\pm$0.13 \\
RAVE J205149.7-615801 & 	--- & 	66 & 	5117$\pm$150 & 	2.87$\pm$0.30 & 	1.17$\pm$0.20 & 	$-$2.03$\pm$0.11 \\
RAVE J205609.1-133118 & 	BD-14 5890, HD 358059 & 	93 & 	4804$\pm$150 & 	1.66$\pm$0.30 & 	1.79$\pm$0.20 & 	$-$2.33$\pm$0.10 \\
RAVE J210634.7-495750 & 	CD-50 13237, HD 200654, NBP 286 & 	150 & 	4934$\pm$150 & 	2.03$\pm$0.30 & 	1.55$\pm$0.20 & 	$-$3.24$\pm$0.06 \\
RAVE J210642.9-682827 & 	--- & 	58 & 	4942$\pm$150 & 	1.93$\pm$0.30 & 	1.65$\pm$0.20 & 	$-$2.95$\pm$0.12 \\
RAVE J211525.5-150331 & 	--- & 	21 & 	4807$\pm$150 & 	1.91$\pm$0.30 & 	2.30$\pm$0.20 & 	$-$2.08$\pm$0.22 \\
RAVE J211927.1-402908 & 	--- & 	52 & 	4686$\pm$150 & 	1.59$\pm$0.30 & 	1.29$\pm$0.20 & 	$-$2.15$\pm$0.12 \\
RAVE J212921.0-620915 & 	--- & 	57 & 	4686$\pm$150 & 	1.33$\pm$0.30 & 	1.59$\pm$0.20 & 	$-$2.46$\pm$0.09 \\
RAVE J215118.3-135937 & 	--- & 	47 & 	4968$\pm$150 & 	2.04$\pm$0.30 & 	1.84$\pm$0.20 & 	$-$1.99$\pm$0.16 \\
RAVE J220211.8-441702 & 	--- & 	61 & 	4953$\pm$150 & 	2.09$\pm$0.30 & 	1.47$\pm$0.20 & 	$-$2.88$\pm$0.09 \\
RAVE J220403.6-402919 & 	--- & 	23 & 	4974$\pm$150 & 	1.91$\pm$0.30 & 	1.80$\pm$0.20 & 	$-$2.57$\pm$0.16 \\
2MASS J22122728-6810067 & 	--- & 	38 & 	4898$\pm$150 & 	2.25$\pm$0.30 & 	1.67$\pm$0.20 & 	$-$1.76$\pm$0.12 \\
RAVE J222236.0-013827 & 	BPS CS 29502-0092 & 	47 & 	5118$\pm$150 & 	2.33$\pm$0.30 & 	2.00$\pm$0.20 & 	$-$2.82$\pm$0.14 \\
RAVE J223716.2-160801 & 	BD-16 6116 & 	42 & 	5959$\pm$150 & 	3.30$\pm$0.30 & 	1.64$\pm$0.20 & 	$-$2.21$\pm$0.10 \\
RAVE J224927.6-223829 & 	--- & 	66 & 	4592$\pm$150 & 	1.14$\pm$0.30 & 	1.87$\pm$0.20 & 	$-$2.03$\pm$0.13 \\
RAVE J225319.9-224856 & 	CD-23 17654 & 	21 & 	4509$\pm$150 & 	1.16$\pm$0.30 & 	2.13$\pm$0.20 & 	$-$2.16$\pm$0.14 \\
RAVE J225926.9-523733 & 	--- & 	46 & 	4948$\pm$150 & 	2.22$\pm$0.30 & 	1.46$\pm$0.20 & 	$-$2.20$\pm$0.11 \\
RAVE J230222.9-683323 & 	--- & 	50 & 	5375$\pm$150 & 	3.03$\pm$0.30 & 	1.95$\pm$0.20 & 	$-$2.26$\pm$0.15 \\
RAVE J231300.0-450707 & 	HE 2310-4523 & 	62 & 	4804$\pm$150 & 	1.45$\pm$0.30 & 	2.71$\pm$0.20 & 	$-$2.53$\pm$0.12 \\
2MASS J23131638-7011223 & 	--- & 	39 & 	4776$\pm$150 & 	1.77$\pm$0.30 & 	1.17$\pm$0.20 & 	$-$2.19$\pm$0.09 \\ 
\enddata
\tablecomments{The stars with 2MASS names don't have RAVE parameters.}
\end{deluxetable*}


==> Table4_LineLists.tex <==
\startlongtable

\begin{deluxetable*}{lllr}
\tablecaption{\label{tab:line_list}Line List for EW Analysis}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Ion}  & 
\colhead{$\lambda$} & 
\colhead{$\chi$} &
\colhead{log $gf$}
}
\startdata
Fe I  & 3963.1  & 3.281 & $-$0.68  \\
Fe I  & 3977.74 & 2.196 & $-$1.12  \\
Fe I  & 4001.66 & 2.174 & $-$1.90  \\
Fe I  & 4005.24 & 1.556 & $-$0.58  \\
Fe I  & 4032.63 & 1.484 & $-$2.38  \\
Fe I  & 4045.81 & 1.484 & 0.28   \\
Fe I  & 4058.22 & 3.209 & $-$1.18  \\
Fe I  & 4063.28 & 3.368 & $-$0.81  \\
Fe I  & 4063.59 & 1.556 & 0.06   \\
Fe I  & 4067.98 & 3.209 & $-$0.53  \\
Fe I  & 4070.77 & 3.239 & $-$0.87  \\
Fe I  & 4071.74 & 1.607 & $-$0.01  \\
Fe I  & 4073.76 & 3.263 & $-$0.97  \\
Fe I  & 4076.63 & 3.209 & $-$0.59  \\
Fe I  & 4080.21 & 3.281 & $-$1.18  \\
Fe I  & 4084.49 & 3.329 & $-$0.54  \\
Fe I  & 4098.18 & 3.239 & $-$0.97  \\
Fe I  & 4127.78 & 3.281 & $-$1.61  \\
Fe I  & 4132.06 & 1.607 & $-$0.68  \\
Fe I  & 4133.86 & 3.366 & $-$1.13  \\
Fe I  & 4139.93 & 0.989 & $-$3.51  \\
Fe I  & 4143.87 & 1.556 & $-$0.51  \\
Fe I  & 4147.67 & 1.484 & $-$2.07  \\
Fe I  & 4150.25 & 3.428 & $-$1.19  \\
Fe I  & 4152.17 & 0.957 & $-$3.16  \\
Fe I  & 4153.9  & 3.397 & $-$0.28  \\
Fe I  & 4158.79 & 3.428 & $-$0.70  \\
Fe I  & 4173.92 & 0.989 & $-$3.29  \\
Fe I  & 4174.91 & 0.914 & $-$2.94  \\
Fe I  & 4187.04 & 2.450  & $-$0.56  \\
Fe I  & 4199.1  & 3.050  & 0.17   \\
Fe I  & 4202.03 & 1.484 & $-$0.69  \\
Fe I  & 4206.7  & 0.052 & $-$3.96  \\
Fe I  & 4216.18 & 0.000     & $-$3.36  \\
Fe I  & 4233.6  & 2.482 & $-$0.60  \\
Fe I  & 4250.79 & 1.556 & $-$0.71  \\
Fe I  & 4258.32 & 0.087 & $-$4.36  \\
Fe I  & 4271.76 & 1.490 & $-$0.17  \\
Fe I  & 4282.4  & 2.174 & $-$0.78  \\
Fe I  & 4291.46 & 0.052 & $-$4.08  \\
Fe I  & 4325.76 & 1.607 & 0.01   \\
Fe I  & 4337.05 & 1.556 & $-$1.70  \\
Fe I  & 4367.9  & 1.607 & $-$2.88  \\
Fe I  & 4375.93 & 0.000     & $-$3.00     \\
Fe I  & 4401.29 & 3.603 & $-$0.99  \\
Fe I  & 4404.75 & 1.556 & $-$0.15  \\
Fe I  & 4408.41 & 2.196 & $-$1.74  \\
Fe I  & 4415.12 & 1.607 & $-$0.62  \\
Fe I  & 4427.31 & 0.052 & $-$2.92  \\
Fe I  & 4442.34 & 2.196 & $-$1.23  \\
Fe I  & 4447.72 & 2.221 & $-$1.36  \\
Fe I  & 4459.12 & 2.174 & $-$1.29  \\
Fe I  & 4461.65 & 0.087 & $-$3.19  \\
Fe I  & 4476.08 & 3.686 & $-$0.34  \\
Fe I  & 4484.22 & 3.600   & $-$0.64  \\
Fe I  & 4489.74 & 0.121 & $-$3.90  \\
Fe I  & 4494.56 & 2.196 & $-$1.14  \\
Fe I  & 4528.61 & 2.174 & $-$0.89  \\
Fe I  & 4531.15 & 1.484 & $-$2.10  \\
Fe I  & 4554.45 & 2.863 & $-$2.81  \\
Fe I  & 4574.22 & 3.209 & $-$2.35  \\
Fe I  & 4592.65 & 1.556 & $-$2.46  \\
Fe I  & 4595.36 & 3.300   & $-$1.73  \\
Fe I  & 4602    & 1.607 & $-$3.13  \\
Fe I  & 4602.94 & 1.484 & $-$2.21  \\
Fe I  & 4607.65 & 3.263 & $-$1.33  \\
Fe I  & 4619.29 & 3.60   & $-$1.06  \\
Fe I  & 4630.12 & 2.277 & $-$2.58  \\
Fe I  & 4637.5  & 3.281 & $-$1.29  \\
Fe I  & 4668.13 & 3.263 & $-$1.08  \\
Fe I  & 4669.17 & 3.651 & $-$1.25  \\
Fe I  & 4678.85 & 3.600   & $-$0.68  \\
Fe I  & 4704.95 & 3.684 & $-$1.32  \\
Fe I  & 4707.27 & 3.241 & $-$0.96  \\
Fe I  & 4709.09 & 3.651 & $-$1.32  \\
Fe I  & 4733.59 & 1.484 & $-$2.99  \\
Fe I  & 4736.77 & 3.209 & $-$0.67  \\
Fe I  & 4741.07 & 3.332 & $-$2.40  \\
Fe I  & 4772.8  & 1.556 & $-$2.90  \\
Fe I  & 4787.83 & 2.996 & $-$2.62  \\
Fe I  & 4807.71 & 3.368 & $-$2.15  \\
Fe I  & 4855.67 & 3.366 & $-$1.63  \\
Fe I  & 4871.32 & 2.865 & $-$0.34  \\
Fe I  & 4875.88 & 3.332 & $-$1.90  \\
Fe I  & 4882.14 & 3.414 & $-$1.48  \\
Fe I  & 4885.43 & 3.882 & $-$0.97  \\
Fe I  & 4890.76 & 2.876 & $-$0.38  \\
Fe I  & 4896.44 & 3.881 & $-$1.89  \\
Fe I  & 4903.31 & 2.882 & $-$0.89  \\
Fe I  & 4905.13 & 3.929 & $-$1.73  \\
Fe I  & 4907.73 & 3.428 & $-$1.70  \\
Fe I  & 4910.02 & 3.394 & $-$1.28  \\
Fe I  & 4911.53 & 4.256 & $-$1.84  \\
Fe I  & 4911.78 & 3.929 & $-$1.75  \\
Fe I  & 4939.69 & 0.858 & $-$3.25  \\
Fe I  & 4946.39 & 3.368 & $-$1.11  \\
Fe I  & 4950.11 & 3.414 & $-$1.50  \\
Fe I  & 4966.09 & 3.329 & $-$0.79  \\
Fe I  & 4973.1  & 3.960  & $-$0.69  \\
Fe I  & 4985.25 & 3.926 & $-$0.44  \\
Fe I  & 4986.94 & 4.256 & $-$1.34  \\
Fe I  & 4994.13 & 0.914 & $-$2.97  \\
Fe I  & 5001.86 & 3.882 & $-$0.01  \\
Fe I  & 5002.79 & 3.397 & $-$1.46  \\
Fe I  & 5005.71 & 3.884 & $-$0.12  \\
Fe I  & 5012.07 & 0.858 & $-$2.60  \\
Fe I  & 5014.94 & 3.940  & $-$0.18  \\
Fe I  & 5022.24 & 3.984 & $-$0.33  \\
Fe I  & 5023.5  & 4.312 & $-$1.67  \\
Fe I  & 5028.13 & 3.570  & $-$1.02  \\
Fe I  & 5039.25 & 3.366 & $-$1.52  \\
Fe I  & 5041.07 & 0.957 & $-$3.09  \\
Fe I  & 5041.76 & 1.484 & $-$2.20  \\
Fe I  & 5048.44 & 3.957 & $-$1.00     \\
Fe I  & 5051.64 & 0.914 & $-$2.76  \\
Fe I  & 5060.08 & 0.000     & $-$5.43  \\
Fe I  & 5079.22 & 2.196 & $-$2.10  \\
Fe I  & 5079.74 & 0.989 & $-$3.25  \\
Fe I  & 5083.34 & 0.957 & $-$2.84  \\
Fe I  & 5110.41 & 0.000     & $-$3.76  \\
Fe I  & 5123.72 & 1.010  & $-$3.06  \\
Fe I  & 5127.36 & 0.914 & $-$3.25  \\
Fe I  & 5129.63 & 3.943 & $-$1.67  \\
Fe I  & 5133.69 & 4.175 & 0.36   \\
Fe I  & 5139.25 & 2.998 & $-$0.73  \\
Fe I  & 5142.93 & 0.957 & $-$3.07  \\
Fe I  & 5150.84 & 0.989 & $-$3.04  \\
Fe I  & 5151.91 & 1.010  & $-$3.32  \\
Fe I  & 5166.28 & 0.000     & $-$4.12  \\
Fe I  & 5168.9  & 0.052 & $-$4.00     \\
Fe I  & 5171.6  & 1.484 & $-$1.72  \\
Fe I  & 5194.94 & 1.556 & $-$2.02  \\
Fe I  & 5202.34 & 2.174 & $-$1.87  \\
Fe I  & 5208.59 & 3.239 & $-$0.89  \\
Fe I  & 5215.18 & 3.263 & $-$0.86  \\
Fe I  & 5216.27 & 1.607 & $-$2.08  \\
Fe I  & 5217.39 & 3.209 & $-$1.07  \\
Fe I  & 5226.86 & 3.038 & $-$0.55  \\
Fe I  & 5227.19 & 1.556 & $-$1.23  \\
Fe I  & 5242.49 & 3.630  & $-$0.83  \\
Fe I  & 5247.05 & 0.087 & $-$4.97  \\
Fe I  & 5250.21 & 0.121 & $-$4.90  \\
Fe I  & 5250.65 & 2.196 & $-$2.18  \\
Fe I  & 5253.46 & 3.281 & $-$1.58  \\
Fe I  & 5254.96 & 0.110  & $-$4.76  \\
Fe I  & 5263.31 & 3.263 & $-$0.87  \\
Fe I  & 5269.54 & 0.858 & -1.33  \\
Fe I  & 5273.16 & 3.289 & -1.01  \\
Fe I  & 5283.62 & 3.239 & -0.45  \\
Fe I  & 5285.13 & 4.435 & -1.66  \\
Fe I  & 5288.52 & 3.695 & -1.49  \\
Fe I  & 5302.3  & 3.281 & -0.73  \\
Fe I  & 5307.36 & 1.607 & -2.91  \\
Fe I  & 5324.18 & 3.211 & -0.11  \\
Fe I  & 5328.04 & 0.914 & -1.47  \\
Fe I  & 5328.53 & 1.556 & -1.85  \\
Fe I  & 5332.9  & 1.556 & -2.78  \\
Fe I  & 5339.93 & 3.263 & -0.63  \\
Fe I  & 5341.02 & 1.607 & -1.95  \\
Fe I  & 5353.37 & 4.103 & -0.76  \\
Fe I  & 5371.49 & 0.957 & -1.64  \\
Fe I  & 5373.71 & 4.473 & -0.71  \\
Fe I  & 5379.57 & 3.690 & -1.42  \\
Fe I  & 5393.17 & 3.241 & -0.72  \\
Fe I  & 5397.13 & 0.914 & -1.98  \\
Fe I  & 5405.78 & 0.989 & -1.85  \\
Fe I  & 5429.7  & 0.957 & -1.88  \\
Fe I  & 5434.52 & 1.010  & -2.13  \\
Fe I  & 5473.9  & 4.154 & -0.72  \\
Fe I  & 5476.56 & 4.100   & -0.28  \\
Fe I  & 5483.1  & 4.151 & -1.39  \\
Fe I  & 5493.5  & 4.103 & -1.48  \\
Fe I  & 5497.52 & 1.010  & -2.83  \\
Fe I  & 5506.78 & 0.989 & -2.79  \\
Fe I  & 5554.9  & 4.549 & -0.27  \\
Fe I  & 5563.6  & 4.191 & -0.75  \\
Fe I  & 5569.62 & 3.414 & -0.52  \\
Fe I  & 5572.84 & 3.394 & -0.28  \\
Fe I  & 5573.1  & 4.188 & -1.29  \\
 & & & \\
Fe II & 4122.67 & 2.580  & $-$3.38  \\
Fe II & 4128.75 & 2.580  & $-$3.47  \\
Fe II & 4173.35 & 2.969 & $-$2.38  \\
Fe II & 4178.86 & 2.580  & $-$2.44  \\
Fe II & 4233.16 & 2.927 & $-$2.02  \\
Fe II & 4303.17 & 2.880  & $-$2.52  \\
Fe II & 4351.76 & 2.848 & $-$1.95  \\
Fe II & 4385.38 & 2.826 & $-$2.64  \\
Fe II & 4416.82 & 2.806 & $-$2.57  \\
Fe II & 4489.18 & 2.828 & $-$2.971 \\
Fe II & 4491.41 & 2.850  & $-$2.64  \\
Fe II & 4508.28 & 2.749 & $-$2.42  \\
Fe II & 4515.34 & 2.840  & $-$2.36  \\
Fe II & 4520.22 & 2.810  & $-$2.60   \\
Fe II & 4522.63 & 2.740  & $-$2.29  \\
Fe II & 4541.52 & 2.860  & $-$2.79  \\
Fe II & 4549.47 & 2.724 & $-$1.92  \\
Fe II & 4555.89 & 2.830  & $-$2.25  \\
Fe II & 4576.34 & 2.840  & $-$2.92  \\
Fe II & 4582.84 & 2.840  & $-$3.06  \\
Fe II & 4583.83 & 2.703 & $-$1.94  \\
Fe II & 4620.52 & 2.830  & $-$3.19  \\
Fe II & 4923.93 & 2.890  & $-$1.21  \\
Fe II & 5018.44 & 2.891 & $-$1.345 \\
Fe II & 5100.66 & 2.807 & $-$4.135 \\
Fe II & 5169.03 & 2.890  & $-$0.87  \\
Fe II & 5197.58 & 3.230  & $-$2.05  \\
Fe II & 5234.63 & 3.220  & $-$2.18  \\
Fe II & 5254.93 & 3.230  & $-$3.336 \\
Fe II & 5264.81 & 3.230  & $-$3.23  \\
Fe II & 5276    & 3.200   & $-$1.90  \\
Fe II & 5284.11 & 2.891 & $-$3.195 \\
Fe II & 5316.62 & 3.150  & $-$1.78  \\
Fe II & 5325.55 & 3.220  & $-$3.16  \\
Fe II & 5362.87 & 3.199 & $-$2.616 \\
Fe II & 5414.07 & 3.220  & $-$3.58  \\
Fe II & 5425.26 & 3.199 & $-$3.39  \\
Fe II & 5534.85 & 3.245 & $-$2.865 \\
& & & \\
Mg I  & 3986.753 & 4.346 & $-$1.03  \\
Mg I  & 4057.505 & 4.346 & $-$0.89  \\
Mg I  & 4167.271 & 4.346 & $-$0.71  \\
Mg I  & 4351.906 & 4.340  & $-$0.525 \\
Mg I  & 4571.096 & 0.000     & $-$5.688 \\
Mg I  & 4702.99  & 4.330  & $-$0.38  \\
Mg I  & 5172.684 & 2.710  & $-$0.45  \\
Mg I  & 5183.604 & 2.720  & $-$0.239 \\
Mg I  & 5528.405 & 4.340  & $-$0.498 \\
 & & & \\
Si I  & 4102.936 & 1.910  & $-$3.14  \\
 & & & \\
Ca I  & 4226.73  & 0.000     & 0.244  \\
Ca I  & 4283.01  & 1.886 & $-$0.224 \\
Ca I  & 4318.65  & 1.890  & $-$0.21  \\
Ca I  & 4425.44  & 1.879 & $-$0.358 \\
Ca I  & 4434.96  & 1.886 & $-$0.01  \\
Ca I  & 4435.69  & 1.890  & $-$0.519 \\
Ca I  & 4454.78  & 1.898 & 0.26   \\
Ca I  & 4455.89  & 1.899 & $-$0.53  \\
Ca I  & 5262.244 & 2.521 & $-$0.471 \\
Ca I  & 5265.556 & 2.520  & $-$0.26  \\
Ca I  & 5349.465 & 2.710  & $-$0.31  \\
 & & & \\
Sc I  & 4995.002 & 2.111 & $-$0.88  \\
 & & & \\
Sc II & 4246.82  & 0.315 & 0.24   \\
Sc II & 4314.083 & 0.620  & $-$0.10   \\
Sc II & 4324.998 & 0.595 & $-$0.44  \\
Sc II & 4400.389 & 0.610  & $-$0.54  \\
Sc II & 4415.544 & 0.595 & $-$0.67  \\
Sc II & 5031.01  & 1.357 & $-$0.40  \\
Sc II & 5239.811 & 1.455 & $-$0.77  \\
Sc II & 5318.374 & 1.357 & $-$2.01  \\
Sc II & 5526.785 & 1.768 & 0.02   \\
 & & & \\
Ti I  & 3989.76  & 0.021 & $-$0.062 \\
Ti I  & 3998.64  & 0.048 & 0.01   \\
Ti I  & 4008.928 & 0.021 & $-$1.016 \\
Ti I  & 4512.73  & 0.840  & $-$0.424 \\
Ti I  & 4518.02  & 0.830  & $-$0.269 \\
Ti I  & 4533.249 & 0.848 & 0.532  \\
Ti I  & 4534.78  & 0.840  & 0.336  \\
Ti I  & 4535.567 & 0.826 & 0.12   \\
Ti I  & 4544.687 & 0.818 & $-$0.52  \\
Ti I  & 4548.76  & 0.830  & $-$0.298 \\
Ti I  & 4555.49  & 0.850  & $-$0.432 \\
Ti I  & 4656.47  & 0.000     & $-$1.289 \\
Ti I  & 4681.91  & 0.048 & $-$1.015 \\
Ti I  & 4840.87  & 0.900  & $-$0.453 \\
Ti I  & 4981.73  & 0.840  & 0.56   \\
Ti I  & 4991.07  & 0.840  & 0.436  \\
Ti I  & 4999.5   & 0.830  & 0.306  \\
Ti I  & 5007.206 & 0.818 & 0.168  \\
Ti I  & 5009.645 & 0.021 & $-$2.203 \\
Ti I  & 5014.187 & 0.000     & $-$1.22  \\
Ti I  & 5014.276 & 0.810  & 0.11   \\
Ti I  & 5016.16  & 0.850  & $-$0.518 \\
Ti I  & 5020.024 & 0.836 & $-$0.358 \\
Ti I  & 5024.843 & 0.818 & $-$0.546 \\
Ti I  & 5035.902 & 1.460  & 0.26   \\
Ti I  & 5036.463 & 1.443 & 0.186  \\
Ti I  & 5038.396 & 1.430  & 0.069  \\
Ti I  & 5039.96  & 0.020  & $-$1.13  \\
Ti I  & 5064.65  & 0.050  & $-$0.935 \\
Ti I  & 5173.74  & 0.000     & $-$1.062 \\
Ti I  & 5192.97  & 0.020  & $-$0.95  \\
Ti I  & 5210.39  & 0.050  & $-$0.828 \\
 & & & \\
Ti II & 4012.396 & 0.574 & $-$1.75  \\
Ti II & 4025.12  & 0.607 & $-$1.98  \\
Ti II & 4028.338 & 1.890  & $-$0.96  \\
Ti II & 4053.829 & 1.893 & $-$1.21  \\
Ti II & 4161.527 & 1.084 & $-$2.16  \\
Ti II & 4163.634 & 2.590  & $-$0.40  \\
Ti II & 4184.309 & 1.080  & $-$2.51  \\
Ti II & 4290.219 & 1.160  & $-$0.93  \\
Ti II & 4300.049 & 1.180  & $-$0.49  \\
Ti II & 4330.723 & 1.180  & $-$2.06  \\
Ti II & 4337.914 & 1.080  & $-$0.96  \\
Ti II & 4394.059 & 1.221 & $-$1.78  \\
Ti II & 4395.031 & 1.080  & $-$0.54  \\
Ti II & 4395.839 & 1.243 & $-$1.93  \\
Ti II & 4398.292 & 1.210  & $-$2.65  \\
Ti II & 4399.765 & 1.240  & $-$1.19  \\
Ti II & 4409.52  & 1.230  & $-$2.37  \\
Ti II & 4417.714 & 1.165 & $-$1.19  \\
Ti II & 4418.331 & 1.240  & $-$1.97  \\
Ti II & 4441.731 & 1.180  & $-$2.41  \\
Ti II & 4443.801 & 1.080  & $-$0.72  \\
Ti II & 4444.554 & 1.120  & $-$2.24  \\
Ti II & 4450.482 & 1.080  & $-$1.52  \\
Ti II & 4464.448 & 1.160  & $-$1.81  \\
Ti II & 4468.517 & 1.131 & $-$0.60  \\
Ti II & 4470.853 & 1.165 & $-$2.02  \\
Ti II & 4488.342 & 3.124 & $-$0.82  \\
Ti II & 4493.522 & 1.080  & $-$3.02  \\
Ti II & 4501.27  & 1.116 & $-$0.77  \\
Ti II & 4529.48  & 1.572 & $-$2.03  \\
Ti II & 4533.96  & 1.240  & $-$0.53  \\
Ti II & 4545.144 & 1.131 & $-$1.81  \\
Ti II & 4563.77  & 1.221 & $-$0.96  \\
Ti II & 4571.971 & 1.572 & $-$0.32  \\
Ti II & 4583.409 & 1.160  & $-$2.92  \\
Ti II & 4589.915 & 1.237 & $-$1.79  \\
Ti II & 4636.32  & 1.160  & $-$3.02  \\
Ti II & 4657.2   & 1.240  & $-$2.24  \\
Ti II & 4708.662 & 1.240  & $-$2.34  \\
Ti II & 4779.979 & 2.048 & $-$1.37  \\
Ti II & 4798.532 & 1.080  & $-$2.68  \\
Ti II & 4805.089 & 2.061 & $-$1.10  \\
Ti II & 4865.61  & 1.116 & $-$2.81  \\
Ti II & 4911.175 & 3.124 & $-$0.34  \\
Ti II & 5005.159 & 1.566 & $-$2.73  \\
Ti II & 5129.156 & 1.890  & $-$1.24  \\
Ti II & 5185.902 & 1.890  & $-$1.49  \\
Ti II & 5188.687 & 1.580  & $-$1.05  \\
Ti II & 5226.538 & 1.570  & $-$1.26  \\
Ti II & 5268.607 & 2.598 & $-$1.62  \\
Ti II & 5336.786 & 1.580  & $-$1.59  \\
Ti II & 5381.021 & 1.570  & $-$1.92  \\
Ti II & 5418.768 & 1.580  & $-$2.00     \\
 & & & \\
Cr I  & 3908.762 & 1.004 & $-$1.00     \\
Cr I  & 4254.332 & 0.000     & $-$0.114 \\
Cr I  & 4274.8   & 0.000     & $-$0.22  \\
Cr I  & 4289.72  & 0.000     & $-$0.37  \\
Cr I  & 4337.566 & 0.968 & $-$1.112 \\
Cr I  & 4545.95  & 0.940  & $-$1.37  \\
Cr I  & 4580.056 & 0.941 & $-$1.65  \\
Cr I  & 4600.752 & 1.004 & $-$1.26  \\
Cr I  & 4616.137 & 0.983 & $-$1.19  \\
Cr I  & 4626.188 & 0.968 & $-$1.32  \\
Cr I  & 4646.15  & 1.030  & $-$0.74  \\
Cr I  & 4651.28  & 0.980  & $-$1.46  \\
Cr I  & 4652.158 & 1.004 & $-$1.03  \\
Cr I  & 4789.34  & 2.540  & $-$0.33  \\
Cr I  & 5206.04  & 0.940  & 0.02   \\
Cr I  & 5208.419 & 0.940  & 0.16   \\
Cr I  & 5247.564 & 0.961 & $-$1.64  \\
Cr I  & 5296.69  & 0.980  & $-$1.36  \\
Cr I  & 5298.28  & 0.980  & $-$1.14  \\
Cr I  & 5300.74  & 0.980  & $-$2.00     \\
Cr I  & 5345.8   & 1.000     & $-$0.95  \\
Cr I  & 5348.31  & 1.000     & $-$1.21  \\
Cr I  & 5409.77  & 1.030  & $-$0.67  \\
& & & \\
Cr II & 4558.594 & 4.070  & $-$0.656 \\
Cr II & 4588.142 & 4.070  & $-$0.826 \\
Cr II & 4591.992 & 4.070  & $-$1.419 \\
 & & & \\
Mn I  & 4030.753 & 0.000     & $-$0.48  \\
Mn I  & 4033.062 & 0.000     & $-$0.618 \\
Mn I  & 4034.483 & 0.000     & $-$0.811 \\
Mn I  & 4041.357 & 2.114 & 0.285  \\
Mn I  & 4754.048 & 2.282 & $-$0.086 \\
Mn I  & 4783.432 & 2.298 & 0.042  \\
Mn I  & 4823.528 & 2.319 & 0.144  \\
 & & & \\
Co I  & 3995.306 & 0.923 & $-$0.22  \\
Co I  & 4020.898 & 0.432 & $-$2.07  \\
Co I  & 4110.532 & 1.049 & $-$1.08  \\
Co I  & 4118.767 & 1.050  & $-$0.49  \\
Co I  & 4121.318 & 0.923 & $-$0.32  \\
 & & & \\
Ni I  & 4605     & 3.480  & $-$0.29  \\
Ni I  & 4648.659 & 3.420  & $-$0.16  \\
Ni I  & 4686.22  & 3.600   & $-$0.64  \\
Ni I  & 4714.421 & 3.380  & 0.23   \\
Ni I  & 4855.414 & 3.542 & 0.00      \\
Ni I  & 4904.41  & 3.540  & $-$0.17  \\
Ni I  & 4980.161 & 3.606 & $-$0.11  \\
Ni I  & 5017.591 & 3.539 & $-$0.08  \\
Ni I  & 5035.374 & 3.635 & 0.29   \\
Ni I  & 5080.523 & 3.655 & 0.13   \\
Ni I  & 5081.11  & 3.850  & 0.30  \\
Ni I  & 5084.08  & 3.680  & 0.03   \\
Ni I  & 5115.4   & 3.830  & $-$0.11  \\
Ni I  & 5137.075 & 1.676 & $-$1.99  \\
Ni I  & 5155.76  & 3.900   & $-$0.09  \\
Ni I  & 5476.9   & 1.830  & $-$0.89  \\
 & & & \\
Zn I  & 4722.15  & 4.030  & $-$0.39  \\
Zn I  & 4810.528 & 4.080  & $-$0.137 \\
 & & & \\
Sr II & 4077.714 & 0.000     & 0.15   \\
Sr II & 4215.524 & 0.000     & $-$0.18  \\
 & & & \\
Ba II & 4554.033 & 0.000     & 0.163  \\
Ba II & 4934.086 & 0.000     & $-$0.16 \\
 & & & \\
Eu II & 4129.72 & 0.000 & 0.22 \\
Eu II & 4205.04 & 0.000 & 0.21 \\
Eu II & 4435.58 & 0.210 & -0.11
\enddata
\end{deluxetable*}

==> Table5_AlphaAbundances.tex <==
\startlongtable

\begin{deluxetable*}{cccccc}
\tablecaption{\label{tab:ab1} Abundances of Alpha Elements}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{NAME}  & 
\colhead{[Mg/Fe]} & 
\colhead{[Si/Fe]} &  
\colhead{[Ca/Fe]} &
\colhead{[Sc/Fe]} & 
\colhead{[Ti/Fe]} \\
&
\colhead{log$\epsilon$(Mg)} &
\colhead{log$\epsilon$(Si)} &
\colhead{log$\epsilon$(Ca)} &
\colhead{log$\epsilon$(Sc)} &
\colhead{log$\epsilon$(Ti)} 
}
\startdata
RAVE J000438.4-540134 & 	 +0.39$\pm$0.30 [4] & 	 +1.06$\pm$0.20 [1] & 	 +0.58$\pm$0.16 [7] & 	 +0.38$\pm$0.34 [4] & 	 +0.43$\pm$0.24 [53] \\	 &   5.61 &   6.19 &   4.54 &   1.15 &   3.00 \\
RAVE J001236.5-181631 & 	 +0.51$\pm$0.24 [6] & 	 +0.67$\pm$0.20 [1] & 	 +0.26$\pm$0.13 [10] & 	 +0.01$\pm$0.13 [4] & 	 +0.25$\pm$0.17 [69] \\	 &   5.70 &   5.77 &   4.19 &   0.75 &   2.79 \\
RAVE J003946.9-684957 & 	 +0.55$\pm$0.10 [4] & 	 ... & 	 +0.60$\pm$0.31 [6] & 	  $-$0.07$\pm$0.10 [2] & 	 +0.32$\pm$0.14 [41] \\	 &   5.53 &  ... &   4.32 &   0.46 &   2.65 \\
RAVE J010839.6-285701 & 	 +0.41$\pm$0.10 [3] & 	 ... & 	 +0.32$\pm$0.11 [2] & 	 +0.01$\pm$0.28 [2] & 	 +0.14$\pm$0.17 [19] \\	 &   5.14 &  ... &   3.79 &   0.29 &   2.22 \\
2MASS J01162885-5343408 & 	 +0.45$\pm$0.13 [8] & 	 +1.17$\pm$0.20 [1] & 	 +0.36$\pm$0.12 [8] & 	 +0.04$\pm$0.24 [4] & 	 +0.33$\pm$0.17 [62] \\	 &   5.29 &   5.92 &   3.94 &   0.43 &   2.52 \\
2MASS J01201051-4849461 & 	 +0.26$\pm$0.10 [3] & 	 ... & 	 +0.46$\pm$0.20 [6] & 	  $-$0.06$\pm$0.10 [3] & 	 +0.30$\pm$0.16 [47] \\	 &   5.69 &  ... &   4.63 &   0.92 &   3.08 \\
RAVE J012931.1-160046 & 	 +0.46$\pm$0.17 [5] & 	 ... & 	 +0.54$\pm$0.10 [7] & 	  $-$0.03$\pm$0.10 [7] & 	 +0.28$\pm$0.20 [53] \\	 &   5.08 &  ... &   3.90 &   0.14 &   2.25 \\
RAVE J013807.0-195210 & 	 +0.21$\pm$0.38 [5] & 	 +1.16$\pm$0.20 [1] & 	 +0.29$\pm$0.20 [6] & 	 +0.23$\pm$0.10 [4] & 	 +0.53$\pm$0.25 [61] \\	 &   5.76 &   6.62 &   4.58 &   1.33 &   3.43 \\
RAVE J014254.2-503249 & 	 +0.33$\pm$0.13 [6] & 	 ... & 	 +0.39$\pm$0.16 [9] & 	 +0.20$\pm$0.23 [7] & 	 +0.35$\pm$0.15 [66] \\	 &   5.75 &  ... &   4.55 &   1.17 &   3.12 \\
RAVE J014908.0-491143 & 	 +0.63$\pm$0.17 [5] & 	 ... & 	 +0.61$\pm$0.13 [8] & 	 +0.01$\pm$0.13 [7] & 	 +0.26$\pm$0.12 [52] \\	 &   5.15 &  ... &   3.87 &   0.08 &   2.13 \\
RAVE J021110.2-191124 & 	 +0.38$\pm$0.24 [7] & 	 +1.05$\pm$0.20 [1] & 	 +0.44$\pm$0.11 [10] & 	 +0.13$\pm$0.27 [7] & 	 +0.35$\pm$0.17 [66] \\	 &   5.61 &   6.19 &   4.41 &   0.91 &   2.93 \\
RAVE J022013.3-601436 & 	 +0.21$\pm$0.27 [4] & 	 +1.09$\pm$0.20 [1] & 	 +0.52$\pm$0.27 [6] & 	 +0.21$\pm$0.24 [4] & 	 +0.32$\pm$0.21 [64] \\	 &   6.14 &   6.93 &   5.19 &   1.69 &   3.60 \\
RAVE J030639.1-692040 & 	 +0.47$\pm$0.11 [4] & 	 ... & 	 +0.59$\pm$0.32 [3] & 	  $-$0.06$\pm$0.10 [4] & 	 +0.25$\pm$0.16 [37] \\	 &   5.28 &  ... &   4.14 &   0.30 &   2.41 \\
2MASS J03135637-6554095 & 	 +0.02$\pm$0.18 [5] & 	 +0.68$\pm$0.20 [1] & 	 +0.32$\pm$0.21 [7] & 	 +0.02$\pm$0.14 [7] & 	 +0.23$\pm$0.20 [65] \\	 &   5.19 &   5.76 &   4.23 &   0.74 &   2.75 \\
RAVE J034228.2-650036 & 	 +0.39$\pm$0.26 [6] & 	 +0.84$\pm$0.20 [1] & 	 +0.70$\pm$0.31 [9] & 	 +0.37$\pm$0.49 [5] & 	 +0.38$\pm$0.21 [72] \\	 &   5.69 &   6.05 &   4.74 &   1.22 &   3.03 \\
2MASS J04042657-2229357 & 	 +0.37$\pm$0.40 [5] & 	 +0.49$\pm$0.20 [1] & 	 +0.57$\pm$0.49 [6] & 	 +0.25$\pm$0.13 [5] & 	 +0.53$\pm$0.26 [55] \\	 &   6.11 &   6.14 &   5.05 &   1.54 &   3.62 \\
RAVE J040658.7-540556 & 	 +0.24$\pm$0.10 [2] & 	 +1.38$\pm$0.20 [1] & 	 +0.28$\pm$0.10 [5] & 	 +0.14$\pm$0.10 [6] & 	 +0.36$\pm$0.18 [34] \\	 &   5.35 &   6.4 &   4.13 &   0.80 &   2.82 \\
RAVE J045322.6-221040 & 	 +0.33$\pm$0.12 [6] & 	 ... & 	 +0.39$\pm$0.10 [9] & 	 +0.23$\pm$0.10 [4] & 	 +0.51$\pm$0.17 [37] \\	 &   5.62 &  ... &   4.42 &   1.07 &   3.15 \\
2MASS J05023178-4540502 & 	 +0.14$\pm$0.24 [2] & 	 ... & 	 +0.33$\pm$0.35 [3] & 	 +0.63$\pm$0.29 [1] & 	 +0.77$\pm$0.21 [35] \\	 &   6.98 &  ... &   5.91 &   3.02 &   4.96 \\
RAVE J050600.7-351056 & 	 +0.09$\pm$0.22 [4] & 	 +0.62$\pm$0.20 [1] & 	 +0.38$\pm$0.10 [4] & 	 +0.01$\pm$0.21 [4] & 	 +0.38$\pm$0.18 [54] \\	 &   5.71 &   6.15 &   4.74 &   1.18 &   3.35 \\
RAVE J050947.6-442317 & 	 +0.67$\pm$0.17 [3] & 	 ... & 	 +0.44$\pm$0.13 [5] & 	 +0.23$\pm$0.10 [3] & 	 +0.46$\pm$0.14 [27] \\	 &   5.77 &  ... &   4.28 &   0.88 &   2.91 \\
RAVE J053817.0-751621 & 	 +0.34$\pm$0.10 [3] & 	 +0.06$\pm$0.20 [1] & 	 +0.49$\pm$0.30 [6] & 	 +0.14$\pm$0.43 [6] & 	 +0.18$\pm$0.18 [67] \\	 &   5.91 &   5.54 &   4.80 &   1.26 &   3.10 \\
2MASS J05510847-5523127 & 	 +0.60$\pm$0.19 [4] & 	 +0.56$\pm$0.20 [1] & 	 +0.60$\pm$0.21 [10] & 	 +0.28$\pm$0.25 [5] & 	 +0.24$\pm$0.13 [61] \\	 &   5.89 &   5.76 &   4.63 &   1.12 &   2.88 \\
RAVE J061950.0-531212 & 	 +0.49$\pm$0.22 [5] & 	 +1.21$\pm$0.20 [1] & 	 +0.33$\pm$0.16 [10] & 	 +0.17$\pm$0.25 [7] & 	 +0.36$\pm$0.18 [65] \\	 &   6.00 &   6.63 &   4.58 &   1.23 &   3.22 \\
2MASS J06340181-4707492 & 	 +0.32$\pm$0.29 [3] & 	 ... & 	 +0.48$\pm$0.25 [7] & 	 +0.04$\pm$0.10 [3] & 	 +0.37$\pm$0.11 [50] \\	 &   5.66 &  ... &   4.56 &   0.93 &   3.06 \\
RAVE J063736.3-692947 & 	  $-$0.34$\pm$0.80 [5] & 	 ... & 	 +0.31$\pm$0.37 [7] & 	 +0.10$\pm$0.26 [5] & 	 +0.47$\pm$0.23 [33] \\	 &   5.59 &  ... &   4.98 &   1.58 &   3.75 \\
RAVE J070520.3-334324 & 	 +0.68$\pm$0.36 [5] & 	 ... & 	 +0.39$\pm$0.10 [6] & 	  $-$0.05$\pm$0.17 [5] & 	 +0.25$\pm$0.15 [63] \\	 &   5.85 &  ... &   4.30 &   0.67 &   2.77 \\
RAVE J074824.3-483141 & 	 +0.31$\pm$0.20 [8] & 	 ... & 	 +0.40$\pm$0.12 [11] & 	 +0.07$\pm$0.10 [8] & 	 +0.29$\pm$0.15 [83] \\	 &   5.90 &  ... &   4.73 &   1.21 &   3.23 \\
RAVE J100709.2-180947 & 	 +0.18$\pm$0.11 [4] & 	 ... & 	 +0.63$\pm$0.37 [7] & 	 +0.47$\pm$0.35 [5] & 	 +0.26$\pm$0.19 [61] \\	 &   5.86 &  ... &   5.05 &   1.70 &   3.29 \\
RAVE J100824.9-231412 & 	 +0.31$\pm$0.10 [4] & 	 ... & 	 +0.73$\pm$0.10 [3] & 	 +0.00$\pm$0.25 [6] & 	 +0.30$\pm$0.21 [46] \\	 &   5.96 &  ... &   5.12 &   1.20 &   3.30 \\
RAVE J101621.6-295952 & 	 +0.46$\pm$0.34 [7] & 	 +0.71$\pm$0.20 [1] & 	 +0.48$\pm$0.22 [8] & 	 +0.27$\pm$0.33 [6] & 	 +0.38$\pm$0.19 [79] \\	 &   5.94 &   6.1 &   4.70 &   1.30 &   3.21 \\
RAVE J112651.4-180530 & 	 +0.43$\pm$0.15 [6] & 	 ... & 	 +0.42$\pm$0.16 [9] & 	 +0.16$\pm$0.10 [5] & 	 +0.24$\pm$0.22 [43] \\	 &   5.51 &  ... &   4.24 &   0.79 &   2.67 \\
RAVE J113508.3-111328 & 	 +0.46$\pm$0.37 [8] & 	 ... & 	 +0.46$\pm$0.28 [11] & 	 +0.30$\pm$0.27 [8] & 	 +0.44$\pm$0.26 [63] \\	 &   6.74 &  ... &   5.48 &   2.13 &   4.07 \\
RAVE J114444.8-112817 & 	 +0.50$\pm$0.14 [8] & 	 ... & 	 +0.43$\pm$0.11 [10] & 	 +0.03$\pm$0.12 [7] & 	 +0.34$\pm$0.10 [71] \\	 &   5.47 &  ... &   4.14 &   0.55 &   2.66 \\
RAVE J115337.3-020037 & 	 +0.12$\pm$0.15 [2] & 	 +0.76$\pm$0.20 [1] & 	 +0.48$\pm$0.21 [4] & 	 +0.07$\pm$0.20 [1] & 	 +0.43$\pm$0.17 [31] \\	 &   5.29 &   5.84 &   4.39 &   0.79 &   2.95 \\
RAVE J115941.7-382043 & 	 +0.35$\pm$0.19 [4] & 	 +0.57$\pm$0.20 [1] & 	 +0.43$\pm$0.14 [8] & 	 +0.43$\pm$0.18 [7] & 	 +0.40$\pm$0.16 [60] \\	 &   6.72 &   6.85 &   5.54 &   2.35 &   4.12 \\
RAVE J123550.1-313111 & 	 +0.38$\pm$0.10 [6] & 	 +1.68$\pm$0.20 [1] & 	 +0.51$\pm$0.12 [8] & 	 +0.30$\pm$0.43 [8] & 	 +0.33$\pm$0.20 [63] \\	 &   5.39 &   6.6 &   4.26 &   0.86 &   2.69 \\
RAVE J115941.7-382043 & 	 +0.45$\pm$0.28 [4] & 	 ... & 	 +0.48$\pm$0.14 [8] & 	 +0.03$\pm$0.10 [5] & 	 +0.47$\pm$0.18 [33] \\	 &   5.78 &  ... &   4.55 &   0.91 &   3.15 \\
RAVE J124718.3-555047 & 	 +0.48$\pm$0.23 [4] & 	 ... & 	 +0.91$\pm$0.33 [4] & 	 +0.33$\pm$0.16 [3] & 	 +0.42$\pm$0.13 [34] \\	 &   6.08 &  ... &   5.25 &   1.48 &   3.37 \\
RAVE J124753.3-390802 & 	 +0.43$\pm$0.10 [4] & 	 ... & 	 +0.57$\pm$0.32 [6] & 	 +0.17$\pm$0.23 [3] & 	 +0.37$\pm$0.21 [54] \\	 &   5.86 &  ... &   4.74 &   1.15 &   3.15 \\
RAVE J125728.3-512522 & 	 +0.56$\pm$0.35 [5] & 	 +0.97$\pm$0.20 [1] & 	 +0.40$\pm$0.19 [7] & 	 +0.09$\pm$0.23 [5] & 	 +0.30$\pm$0.15 [56] \\	 &   5.69 &   6.01 &   4.27 &   0.77 &   2.78 \\
RAVE J125807.3-450627 & 	 +0.31$\pm$0.28 [5] & 	 ... & 	 +0.30$\pm$0.35 [6] & 	 +0.31$\pm$0.10 [4] & 	 +0.55$\pm$0.24 [56] \\	 &   5.84 &  ... &   4.57 &   1.39 &   3.43 \\
RAVE J130231.2-144805 & 	 +0.44$\pm$0.15 [6] & 	 ... & 	 +0.47$\pm$0.11 [10] & 	 +0.12$\pm$0.10 [7] & 	 +0.38$\pm$0.13 [59] \\	 &   6.29 &  ... &   5.06 &   1.52 &   3.58 \\
RAVE J130404.1-240837 & 	 +0.37$\pm$0.16 [5] & 	 ... & 	 +0.44$\pm$0.21 [6] & 	 +0.10$\pm$0.10 [4] & 	 +0.43$\pm$0.19 [74] \\	 &   5.80 &  ... &   4.61 &   1.08 &   3.21 \\
RAVE J130455.0-371249 & 	 +0.14$\pm$0.20 [3] & 	 ... & 	 +0.26$\pm$0.17 [6] & 	 +0.17$\pm$0.12 [4] & 	 +0.20$\pm$0.11 [38] \\	 &   6.85 &  ... &   5.71 &   2.43 &   4.26 \\
RAVE J133352.8-262354 & 	 +0.50$\pm$0.23 [6] & 	 +1.10$\pm$0.20 [1] & 	 +0.38$\pm$0.14 [7] & 	  $-$0.08$\pm$0.13 [4] & 	 +0.26$\pm$0.15 [60] \\	 &   5.83 &   6.34 &   4.45 &   0.80 &   2.94 \\
RAVE J134723.7-314409 & 	 +0.55$\pm$0.19 [4] & 	 ... & 	 +0.41$\pm$0.18 [8] & 	 +0.24$\pm$0.32 [5] & 	 +0.28$\pm$0.16 [59] \\	 &   6.16 &  ... &   4.76 &   1.40 &   3.24 \\
RAVE J135735.4-303249 & 	 +0.46$\pm$0.14 [6] & 	 ... & 	 +0.40$\pm$0.16 [6] & 	  $-$0.03$\pm$0.14 [5] & 	 +0.40$\pm$0.14 [64] \\	 &   5.60 &  ... &   4.28 &   0.66 &   2.89 \\
RAVE J140329.0-525043 & 	 +0.78$\pm$0.32 [4] & 	 +0.65$\pm$0.20 [1] & 	 +0.45$\pm$0.15 [9] & 	 +0.28$\pm$0.40 [4] & 	 +0.32$\pm$0.14 [54] \\	 &   6.45 &   6.23 &   4.86 &   1.50 &   3.34 \\
RAVE J140335.4-333526 & 	 +0.42$\pm$0.10 [5] & 	 +0.57$\pm$0.20 [1] & 	 +0.55$\pm$0.10 [8] & 	 +0.03$\pm$0.13 [3] & 	 +0.35$\pm$0.13 [25] \\	 &   5.27 &   5.33 &   4.14 &   0.43 &   2.55 \\
RAVE J141126.2-113746 & 	 +0.28$\pm$0.19 [4] & 	 ... & 	 +0.24$\pm$0.36 [2] & 	  $-$0.10$\pm$0.17 [4] & 	 +0.88$\pm$0.14 [35] \\	 &   5.13 &  ... &   3.83 &   0.30 &   3.08 \\
RAVE J141253.2-355256 & 	 +0.66$\pm$0.18 [6] & 	 ... & 	 +0.67$\pm$0.16 [8] & 	 +0.08$\pm$0.18 [5] & 	 +0.31$\pm$0.15 [60] \\	 &   5.81 &  ... &   4.56 &   0.78 &   2.81 \\
RAVE J153830.9-180424 & 	 +0.61$\pm$0.28 [8] & 	 +0.81$\pm$0.20 [1] & 	 +0.52$\pm$0.28 [9] & 	 +0.28$\pm$0.37 [8] & 	 +0.38$\pm$0.30 [84] \\	 &   6.01 &   6.12 &   4.66 &   1.23 &   3.13 \\
RAVE J155211.1-143037 & 	 +0.37$\pm$0.20 [6] & 	 ... & 	 +0.34$\pm$0.11 [10] & 	 +0.20$\pm$0.13 [8] & 	 +0.44$\pm$0.20 [74] \\	 &   6.37 &  ... &   5.08 &   1.75 &   3.79 \\
RAVE J155829.6-122434 & 	 +0.58$\pm$0.11 [7] & 	 +0.86$\pm$0.20 [1] & 	 +0.57$\pm$0.16 [11] & 	 +0.10$\pm$0.10 [8] & 	 +0.37$\pm$0.12 [76] \\	 &   5.36 &   5.55 &   4.09 &   0.43 &   2.50 \\
RAVE J160245.0-152102 & 	 +0.41$\pm$0.14 [6] & 	 ... & 	 +0.44$\pm$0.14 [10] & 	 +0.12$\pm$0.10 [7] & 	 +0.34$\pm$0.11 [73] \\	 &   5.96 &  ... &   4.73 &   1.22 &   3.24 \\
RAVE J161847.0-014540 & 	 +0.59$\pm$0.28 [5] & 	 ... & 	 +0.56$\pm$0.23 [6] & 	 +0.19$\pm$0.23 [4] & 	 +0.27$\pm$0.17 [62] \\	 &   6.10 &  ... &   4.81 &   1.25 &   3.13 \\
RAVE J161943.1-022431 & 	 +0.47$\pm$0.15 [3] & 	 ... & 	 +0.47$\pm$0.18 [6] & 	 +0.29$\pm$0.28 [5] & 	 +0.34$\pm$0.13 [58] \\	 &   5.83 &  ... &   4.57 &   1.20 &   3.05 \\
RAVE J165300.5-005507 & 	 +0.57$\pm$0.36 [7] & 	 +0.64$\pm$0.20 [1] & 	 +0.78$\pm$0.55 [11] & 	 +0.40$\pm$0.47 [9] & 	 +0.47$\pm$0.28 [80] \\	 &   6.54 &   6.52 &   5.49 &   1.92 &   3.79 \\
2MASS J17163340-7009028 & 	 +0.43$\pm$0.19 [3] & 	 ... & 	 +0.42$\pm$0.22 [4] & 	 +0.08$\pm$0.15 [6] & 	 +0.33$\pm$0.14 [55] \\	 &   5.34 &  ... &   4.07 &   0.54 &   2.59 \\
RAVE J175159.8-475131 & 	 +0.37$\pm$0.27 [6] & 	 +1.06$\pm$0.20 [1] & 	 +0.37$\pm$0.28 [5] & 	 +0.30$\pm$0.10 [4] & 	 +0.43$\pm$0.13 [52] \\	 &   5.77 &   6.37 &   4.51 &   1.25 &   3.18 \\
RAVE J180242.3-440443 & 	 +0.39$\pm$0.10 [3] & 	 ... & 	 +0.85$\pm$0.34 [3] & 	 +0.11$\pm$0.10 [3] & 	 +0.32$\pm$0.19 [49] \\	 &   6.11 &  ... &   5.31 &   1.38 &   3.39 \\
RAVE J183108.2-491105 & 	 +0.28$\pm$0.20 [6] & 	 +0.14$\pm$0.20 [1] & 	 +0.14$\pm$0.15 [5] & 	  $-$0.06$\pm$0.10 [6] & 	 +0.29$\pm$0.17 [58] \\	 &   5.80 &   5.57 &   4.40 &   1.01 &   3.16 \\
RAVE J183623.2-642812 & 	 +0.39$\pm$0.10 [4] & 	 ... & 	 +0.45$\pm$0.16 [6] & 	 +0.12$\pm$0.16 [5] & 	 +0.30$\pm$0.09 [37] \\	 &   5.45 &  ... &   4.25 &   0.73 &   2.71 \\
2MASS J19031845-5138510 & 	 +0.21$\pm$0.25 [4] & 	 ... & 	 +0.31$\pm$0.20 [1] & 	 +0.24$\pm$0.10 [4] & 	 +0.38$\pm$0.21 [49] \\	 &   5.66 &  ... &   4.50 &   1.24 &   3.18 \\
RAVE J190733.1-415832 & 	 +0.46$\pm$0.10 [4] & 	 ... & 	  $-$0.42$\pm$0.24 [4] & 	 +0.27$\pm$0.28 [4] & 	 +0.33$\pm$0.13 [44] \\	 &   5.62 &  ... &   3.48 &   0.98 &   2.84 \\
RAVE J190923.1-435357 & 	 +0.56$\pm$0.11 [5] & 	 ... & 	 +0.61$\pm$0.41 [3] & 	  $-$0.02$\pm$0.18 [5] & 	 +0.28$\pm$0.11 [39] \\	 &   6.11 &  ... &   4.90 &   1.08 &   3.18 \\
RAVE J191755.9-544015 & 	 +0.56$\pm$0.18 [8] & 	 +0.80$\pm$0.20 [1] & 	 +0.45$\pm$0.14 [10] & 	 +0.09$\pm$0.24 [8] & 	 +0.24$\pm$0.16 [82] \\	 &   5.35 &   5.5 &   3.98 &   0.43 &   2.38 \\
RAVE J192325.2-583341 & 	 +0.35$\pm$0.10 [3] & 	 +0.55$\pm$0.20 [1] & 	 +0.45$\pm$0.16 [5] & 	 +0.18$\pm$0.33 [5] & 	 +0.33$\pm$0.14 [61] \\	 &   5.54 &   5.65 &   4.38 &   0.92 &   2.87 \\
RAVE J192819.9-633935 & 	 +0.62$\pm$0.24 [8] & 	 +0.82$\pm$0.20 [1] & 	 +0.46$\pm$0.14 [11] & 	 +0.32$\pm$0.42 [8] & 	 +0.36$\pm$0.18 [83] \\	 &   5.82 &   5.93 &   4.40 &   1.07 &   2.91 \\
RAVE J193102.8-440158 & 	 +0.49$\pm$0.17 [7] & 	 +0.91$\pm$0.20 [1] & 	 +0.56$\pm$0.25 [6] & 	 +0.04$\pm$0.10 [4] & 	 +0.31$\pm$0.15 [68] \\	 &   5.81 &   6.14 &   4.62 &   0.91 &   2.98 \\
RAVE J194318.7-594820 & 	 +0.09$\pm$0.21 [4] & 	 ... & 	 +0.21$\pm$0.18 [7] & 	 +0.01$\pm$0.16 [4] & 	 +0.31$\pm$0.17 [52] \\	 &   5.52 &  ... &   4.38 &   0.99 &   3.09 \\
RAVE J194319.0-405425 & 	 +0.61$\pm$0.35 [5] & 	 ... & 	 +0.47$\pm$0.10 [8] & 	 +0.11$\pm$0.10 [6] & 	 +0.37$\pm$0.11 [61] \\	 &   6.49 &  ... &   5.09 &   1.54 &   3.60 \\
RAVE J194550.6-392631 & 	 +0.60$\pm$0.16 [8] & 	 +0.83$\pm$0.20 [1] & 	 +0.56$\pm$0.16 [10] & 	 +0.27$\pm$0.25 [9] & 	 +0.36$\pm$0.13 [78] \\	 &   5.23 &   5.37 &   3.93 &   0.45 &   2.34 \\
RAVE J200034.7-342004 & 	 +0.35$\pm$0.25 [3] & 	 +1.11$\pm$0.20 [1] & 	 +0.37$\pm$0.14 [8] & 	 +0.07$\pm$0.18 [5] & 	 +0.31$\pm$0.13 [44] \\	 &   5.83 &   6.5 &   4.59 &   1.10 &   3.14 \\
RAVE J200057.7-254149 & 	 +0.63$\pm$0.23 [7] & 	 +0.87$\pm$0.20 [1] & 	 +0.54$\pm$0.26 [4] & 	 +0.07$\pm$0.10 [4] & 	 +0.37$\pm$0.22 [65] \\	 &   6.14 &   6.29 &   4.79 &   1.13 &   3.23 \\
RAVE J201007.1-515502 & 	 +0.57$\pm$0.10 [6] & 	 +0.24$\pm$0.20 [1] & 	 +0.47$\pm$0.24 [6] & 	  $-$0.05$\pm$0.20 [9] & 	 +0.19$\pm$0.14 [71] \\	 &   5.61 &   5.19 &   4.25 &   0.54 &   2.58 \\
RAVE J202029.2-270735 & 	 +0.55$\pm$0.11 [4] & 	 ... & 	 +0.27$\pm$0.20 [1] & 	  $-$0.07$\pm$0.14 [4] & 	 +0.19$\pm$0.11 [29] \\	 &   5.14 &  ... &   3.60 &   0.07 &   2.13 \\
RAVE J202432.1-151029 & 	 +0.36$\pm$0.11 [6] & 	 +1.22$\pm$0.20 [1] & 	 +0.56$\pm$0.35 [5] & 	 +0.22$\pm$0.15 [6] & 	 +0.44$\pm$0.21 [65] \\	 &   6.25 &   7.02 &   5.19 &   1.66 &   3.68 \\
RAVE J202434.5-423334 & 	 +0.29$\pm$0.17 [4] & 	 ... & 	 +0.15$\pm$0.10 [6] & 	  $-$0.01$\pm$0.15 [7] & 	 +0.24$\pm$0.15 [36] \\	 &   5.21 &  ... &   3.81 &   0.46 &   2.51 \\
2MASS J20264253-1656467 & 	 +0.34$\pm$0.24 [7] & 	 +0.77$\pm$0.20 [1] & 	 +0.49$\pm$0.39 [10] & 	 +0.25$\pm$0.16 [6] & 	 +0.34$\pm$0.14 [67] \\	 &   5.97 &   6.31 &   4.86 &   1.43 &   3.32 \\
RAVE J202654.7-595013 & 	 +0.40$\pm$0.33 [7] & 	 +1.21$\pm$0.20 [1] & 	 +0.57$\pm$0.27 [6] & 	 +0.35$\pm$0.39 [6] & 	 +0.38$\pm$0.15 [65] \\	 &   5.95 &   6.67 &   4.86 &   1.45 &   3.28 \\
RAVE J203428.4-241830 & 	 +0.24$\pm$0.10 [5] & 	 +0.84$\pm$0.20 [1] & 	 +0.34$\pm$0.17 [10] & 	  $-$0.10$\pm$0.16 [6] & 	 +0.10$\pm$0.18 [63] \\	 &   5.36 &   5.87 &   4.20 &   0.57 &   2.57 \\
RAVE J203622.6-071420 & 	 +0.41$\pm$0.18 [4] & 	 ... & 	 +0.62$\pm$0.42 [6] & 	 +0.13$\pm$0.10 [4] & 	 +0.37$\pm$0.16 [46] \\	 &   5.42 &  ... &   4.37 &   0.69 &   2.73 \\
RAVE J203706.4-122125 & 	 +0.50$\pm$0.24 [6] & 	 +0.77$\pm$0.20 [1] & 	 +0.40$\pm$0.20 [7] & 	  $-$0.01$\pm$0.10 [4] & 	 +0.26$\pm$0.15 [56] \\	 &   5.49 &   5.67 &   4.13 &   0.53 &   2.60 \\
RAVE J204355.8-563629 & 	 +0.61$\pm$0.39 [5] & 	 +0.62$\pm$0.20 [1] & 	 +0.48$\pm$0.22 [7] & 	 +0.04$\pm$0.10 [6] & 	 +0.27$\pm$0.17 [65] \\	 &   6.14 &   6.06 &   4.75 &   1.12 &   3.15 \\
RAVE J204450.7-371400 & 	 +0.36$\pm$0.23 [3] & 	 ... & 	 +0.33$\pm$0.25 [5] & 	  $-$0.05$\pm$0.24 [4] & 	 +0.27$\pm$0.11 [32] \\	 &   5.24 &  ... &   3.95 &   0.38 &   2.50 \\
RAVE J204954.4-480045 & 	 +0.72$\pm$0.22 [5] & 	 +0.98$\pm$0.20 [1] & 	 +0.41$\pm$0.20 [9] & 	 +0.29$\pm$0.35 [7] & 	 +0.29$\pm$0.13 [70] \\	 &   6.50 &   6.67 &   4.93 &   1.62 &   3.42 \\
RAVE J205149.7-615801 & 	 +0.35$\pm$0.10 [6] & 	 +1.01$\pm$0.20 [1] & 	 +0.42$\pm$0.23 [11] & 	 +0.01$\pm$0.10 [6] & 	 +0.30$\pm$0.15 [76] \\	 &   5.92 &   6.49 &   4.73 &   1.13 &   3.22 \\
RAVE J205609.1-133118 & 	 +0.43$\pm$0.12 [8] & 	 +0.83$\pm$0.20 [1] & 	 +0.40$\pm$0.17 [11] & 	 +0.21$\pm$0.44 [9] & 	 +0.26$\pm$0.14 [83] \\	 &   5.70 &   6.01 &   4.41 &   1.03 &   2.88 \\
RAVE J210634.7-495750 & 	 +0.55$\pm$0.10 [8] & 	 +0.89$\pm$0.20 [1] & 	 +0.49$\pm$0.11 [9] & 	 +0.11$\pm$0.10 [4] & 	 +0.32$\pm$0.09 [49] \\	 &   4.91 &   5.16 &   3.59 &   0.02 &   2.03 \\
RAVE J210642.9-682827 & 	 +0.43$\pm$0.11 [8] & 	 +1.11$\pm$0.20 [1] & 	 +0.46$\pm$0.17 [11] & 	 +0.08$\pm$0.11 [7] & 	 +0.37$\pm$0.19 [71] \\	 &   5.08 &   5.67 &   3.85 &   0.28 &   2.37 \\
RAVE J211525.5-150331 & 	 +0.26$\pm$0.20 [3] & 	 ... & 	 +0.27$\pm$0.32 [5] & 	 +0.52$\pm$0.53 [4] & 	 +0.29$\pm$0.15 [32] \\	 &   5.78 &  ... &   4.53 &   1.59 &   3.16 \\
RAVE J211927.1-402908 & 	 +0.40$\pm$0.14 [5] & 	 +0.31$\pm$0.20 [1] & 	 +0.58$\pm$0.31 [8] & 	 +0.29$\pm$0.36 [6] & 	 +0.31$\pm$0.19 [68] \\	 &   5.85 &   5.67 &   4.77 &   1.29 &   3.11 \\
RAVE J212921.0-620915 & 	 +0.67$\pm$0.34 [6] & 	 +0.85$\pm$0.20 [1] & 	 +0.63$\pm$0.14 [8] & 	 +0.12$\pm$0.30 [7] & 	 +0.30$\pm$0.14 [67] \\	 &   5.81 &   5.9 &   4.51 &   0.81 &   2.79 \\
RAVE J215118.3-135937 & 	 +0.31$\pm$0.10 [4] & 	 ... & 	 +0.58$\pm$0.22 [7] & 	 +0.32$\pm$0.32 [3] & 	 +0.44$\pm$0.22 [36] \\	 &   5.92 &  ... &   4.93 &   1.48 &   3.40 \\
RAVE J220211.8-441702 & 	 +0.31$\pm$0.11 [6] & 	 ... & 	 +0.31$\pm$0.15 [8] & 	  $-$0.13$\pm$0.10 [6] & 	 +0.29$\pm$0.10 [48] \\	 &   5.03 &  ... &   3.77 &   0.14 &   2.36 \\
RAVE J220403.6-402919 & 	 +0.27$\pm$0.20 [3] & 	 ... & 	 +0.33$\pm$0.17 [4] & 	  $-$0.08$\pm$0.14 [3] & 	 +0.25$\pm$0.12 [25] \\	 &   5.30 &  ... &   4.10 &   0.50 &   2.63 \\
2MASS J22122728-6810067 & 	 +0.13$\pm$0.27 [1] & 	 ... & 	 +0.26$\pm$0.17 [2] & 	 +0.15$\pm$0.10 [2] & 	 +0.31$\pm$0.16 [51] \\	 &   5.97 &  ... &   4.84 &   1.54 &   3.50 \\
RAVE J222236.0-013827 & 	 +0.12$\pm$0.10 [3] & 	 ... & 	 +0.34$\pm$0.26 [6] & 	 +0.26$\pm$0.10 [3] & 	 +0.29$\pm$0.29 [26] \\	 &   4.90 &  ... &   3.86 &   0.59 &   2.42 \\
RAVE J223716.2-160801 & 	 +0.50$\pm$0.37 [8] & 	 ... & 	 +0.41$\pm$0.18 [11] & 	 +0.37$\pm$0.36 [8] & 	 +0.46$\pm$0.17 [57] \\	 &   5.89 &  ... &   4.54 &   1.31 &   3.20 \\
RAVE J224927.6-223829 & 	 +0.51$\pm$0.16 [4] & 	 ... & 	 +0.72$\pm$0.36 [7] & 	 +0.04$\pm$0.10 [3] & 	 +0.36$\pm$0.19 [49] \\	 &   6.08 &  ... &   5.03 &   1.16 &   3.28 \\
RAVE J225319.9-224856 & 	 +0.37$\pm$0.10 [3] & 	 +0.92$\pm$0.20 [1] & 	 +0.53$\pm$0.30 [4] & 	 +0.37$\pm$0.18 [4] & 	 +0.26$\pm$0.11 [39] \\	 &   5.81 &   6.27 &   4.71 &   1.36 &   3.05 \\
RAVE J225926.9-523733 & 	 +0.56$\pm$0.23 [6] & 	 +1.25$\pm$0.20 [1] & 	 +0.42$\pm$0.11 [9] & 	 +0.10$\pm$0.13 [6] & 	 +0.26$\pm$0.16 [72] \\	 &   5.96 &   6.56 &   4.56 &   1.05 &   3.01 \\
RAVE J230222.9-683323 & 	 +0.38$\pm$0.19 [7] & 	 ... & 	 +0.28$\pm$0.13 [7] & 	 +0.19$\pm$0.10 [5] & 	 +0.32$\pm$0.13 [49] \\	 &   5.72 &  ... &   4.36 &   1.08 &   3.01 \\
RAVE J231300.0-450707 & 	 +0.11$\pm$0.15 [5] & 	 +0.83$\pm$0.20 [1] & 	 +0.27$\pm$0.14 [3] & 	  $-$0.25$\pm$0.10 [4] & 	 +0.13$\pm$0.19 [42] \\	 &   5.18 &   5.81 &   4.08 &   0.37 &   2.55 \\
2MASS J23131638-7011223 & 	 +0.21$\pm$0.10 [5] & 	 ... & 	 +0.36$\pm$0.18 [7] & 	 +0.20$\pm$0.24 [5] & 	 +0.26$\pm$0.16 [65] \\	 &   5.62 &  ... &   4.51 &   1.16 &   3.02 \\
\enddata
\end{deluxetable*}

==> Table6_FePeakAbundances.tex <==
\startlongtable

\begin{deluxetable*}{ccccccc}
\tablecaption{\label{tab:ab2} Abundances of Iron-Peak Elements}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{NAME}  & 
\colhead{[Cr/Fe]} & 
\colhead{[Mn/Fe]} &  
\colhead{[Co/Fe]} &
\colhead{[Fe/H]} &
\colhead{[Ni/Fe]} & 
\colhead{[Zn/Fe]} \\
&
\colhead{log$\epsilon$(Cr)} &
\colhead{log$\epsilon$(Mn)} &
\colhead{log$\epsilon$(Co)} &
\colhead{log$\epsilon$(Fe)} &
\colhead{log$\epsilon$(Ni)} &
\colhead{log$\epsilon$(Zn)} 
}
\startdata
RAVE J000438.4-540134 & 	  $-$0.09$\pm$0.09 [11]  & 	  $-$0.38$\pm$0.10 [3]  & 	 ...  & 	  $-$2.38$\pm$0.10 [74]  & 	 +0.05$\pm$0.12 [8]  & 	 +0.21$\pm$0.10 [2]  \\	 &   3.17 &   2.67 &  ... &   5.12 &   3.89 &   2.39 \\
RAVE J001236.5-181631 & 	  $-$0.14$\pm$0.14 [20]  & 	 +0.06$\pm$0.35 [7]  & 	 +0.62$\pm$0.31 [4]  & 	  $-$2.41$\pm$0.09 [106]  & 	 +0.16$\pm$0.10 [14]  & 	 +0.12$\pm$0.10 [2]  \\	 &   3.09 &   3.08 &   3.2 &   5.09 &   3.97 &   2.27 \\
RAVE J003946.9-684957 & 	  $-$0.17$\pm$0.15 [8]  & 	  $-$0.47$\pm$0.20 [1]  & 	 +0.52$\pm$0.2 [1]  & 	  $-$2.62$\pm$0.10 [79]  & 	 +0.09$\pm$0.10 [5]  & 	 +0.27$\pm$0.11 [2]  \\	 &   2.85 &   2.34 &   2.89 &   4.88 &   3.69 &   2.21 \\
RAVE J010839.6-285701 & 	  $-$0.31$\pm$0.24 [5]  & 	 ...  & 	 ...  & 	  $-$2.87$\pm$0.14 [77]  & 	 +0.04$\pm$0.16 [3]  & 	 +0.03$\pm$0.20 [1]  \\	 &   2.46 &  ... &  ... &   4.63 &   3.39 &   1.72 \\
2MASS J01162885-5343408 & 	  $-$0.50$\pm$0.22 [16]  & 	  $-$0.30$\pm$0.53 [6]  & 	 +0.03$\pm$0.27 [2]  & 	  $-$2.76$\pm$0.14 [104]  & 	 +0.09$\pm$0.19 [7]  & 	 +0.06$\pm$0.20 [1]  \\	 &   2.38 &   2.37 &   2.77 &   4.74 &   3.55 &   1.86 \\
2MASS J01201051-4849461 & 	  $-$0.08$\pm$0.12 [8]  & 	  $-$0.38$\pm$0.10 [3]  & 	 ...  & 	  $-$2.17$\pm$0.14 [103]  & 	 +0.07$\pm$0.10 [9]  & 	 +0.19$\pm$0.12 [2]  \\	 &   3.39 &   2.88 &  ... &   5.33 &   4.12 &   2.58 \\
RAVE J012931.1-160046 & 	  $-$0.19$\pm$0.18 [11]  & 	  $-$0.31$\pm$0.20 [1]  & 	 +0.52$\pm$0.2 [1]  & 	  $-$2.98$\pm$0.15 [112]  & 	 +0.16$\pm$0.12 [6]  & 	 +0.14$\pm$0.26 [2]  \\	 &   2.47 &   2.14 &   2.53 &   4.52 &   3.40 &   1.72 \\
RAVE J013807.0-195210 & 	  $-$0.20$\pm$0.17 [12]  & 	  $-$0.23$\pm$0.23 [4]  & 	  $-$0.36$\pm$0.19 [2]  & 	  $-$2.05$\pm$0.14 [87]  & 	 +0.10$\pm$0.21 [10]  & 	 +0.27$\pm$0.10 [2]  \\	 &   3.39 &   3.15 &   3.18 &   5.45 &   4.27 &   2.78 \\
RAVE J014254.2-503249 & 	  $-$0.09$\pm$0.15 [22]  & 	  $-$0.39$\pm$0.10 [3]  & 	 +1.1$\pm$0.2 [1]  & 	  $-$2.18$\pm$0.11 [108]  & 	 +0.04$\pm$0.11 [15]  & 	 +0.25$\pm$0.12 [2]  \\	 &   3.37 &   2.86 &   3.91 &   5.32 &   4.08 &   2.63 \\
RAVE J014908.0-491143 & 	  $-$0.17$\pm$0.13 [13]  & 	  $-$0.24$\pm$0.18 [5]  & 	 +0.94$\pm$0.1 [2]  & 	  $-$3.08$\pm$0.10 [105]  & 	 +0.18$\pm$0.14 [10]  & 	 +0.29$\pm$0.20 [1]  \\	 &   2.39 &   2.11 &   2.85 &   4.42 &   3.32 &   1.77 \\
RAVE J021110.2-191124 & 	  $-$0.07$\pm$0.13 [22]  & 	  $-$0.10$\pm$0.36 [5]  & 	 +0.49$\pm$0.29 [3]  & 	  $-$2.37$\pm$0.10 [111]  & 	 +0.05$\pm$0.14 [13]  & 	  $-$0.01$\pm$0.10 [2]  \\	 &   3.2 &   2.96 &   3.11 &   5.13 &   3.90 &   2.18 \\
RAVE J022013.3-601436 & 	  $-$0.07$\pm$0.13 [18]  & 	  $-$0.13$\pm$0.23 [4]  & 	 +0.44$\pm$0.2 [1]  & 	  $-$1.67$\pm$0.14 [106]  & 	  $-$0.13$\pm$0.12 [13]  & 	  $-$0.06$\pm$0.10 [2]  \\	 &   3.9 &   3.63 &   3.76 &   5.83 &   4.42 &   2.83 \\
RAVE J030639.1-692040 & 	 ...  & 	  $-$0.47$\pm$0.10 [2]  & 	 ...  & 	  $-$2.79$\pm$0.13 [90]  & 	 +0.08$\pm$0.12 [3]  & 	 +0.34$\pm$0.10 [2]  \\	 &  ... &   2.17 &  ... &   4.71 &   3.51 &   2.11 \\
2MASS J03135637-6554095 & 	  $-$0.20$\pm$0.28 [17]  & 	  $-$0.34$\pm$0.15 [3]  & 	 +0.08$\pm$0.25 [2]  & 	  $-$2.43$\pm$0.14 [94]  & 	 +0.08$\pm$0.15 [12]  & 	 +0.20$\pm$0.10 [2]  \\	 &   3.01 &   2.66 &   2.64 &   5.07 &   3.87 &   2.33 \\
RAVE J034228.2-650036 & 	  $-$0.16$\pm$0.09 [19]  & 	  $-$0.02$\pm$0.12 [6]  & 	 +0.27$\pm$0.15 [2]  & 	  $-$2.30$\pm$0.10 [107]  & 	 +0.04$\pm$0.11 [15]  & 	 +0.20$\pm$0.10 [2]  \\	 &   3.18 &   3.11 &   2.96 &   5.20 &   3.96 &   2.46 \\
2MASS J04042657-2229357 & 	 +0.01$\pm$0.25 [14]  & 	  $-$0.16$\pm$0.10 [3]  & 	 ...  & 	  $-$1.86$\pm$0.16 [82]  & 	 +0.17$\pm$0.21 [14]  & 	 +0.33$\pm$0.10 [2]  \\	 &   3.79 &   3.41 &  ... &   5.64 &   4.53 &   3.03 \\
RAVE J040658.7-540556 & 	  $-$0.18$\pm$0.14 [9]  & 	  $-$0.47$\pm$0.13 [3]  & 	 +0.58$\pm$0.2 [1]  & 	  $-$2.49$\pm$0.12 [93]  & 	 +0.11$\pm$0.21 [4]  & 	 +0.24$\pm$0.12 [2]  \\	 &   2.97 &   2.47 &   3.08 &   5.01 &   3.84 &   2.31 \\
RAVE J045322.6-221040 & 	 +0.08$\pm$0.25 [8]  & 	  $-$0.42$\pm$0.10 [4]  & 	 +0.29$\pm$0.1 [2]  & 	  $-$2.31$\pm$0.10 [65]  & 	 +0.24$\pm$0.13 [4]  & 	 ...  \\	 &   3.41 &   2.7 &   3.32 &   5.19 &   4.15 &  ....00 \\
2MASS J05023178-4540502 & 	 +0.23$\pm$0.13 [14]  & 	 +0.15$\pm$0.10 [4]  & 	  $-$0.73$\pm$0.2 [1]  & 	  $-$0.76$\pm$0.17 [57]  & 	 +0.17$\pm$0.62 [10]  & 	 +0.31$\pm$0.11 [2]  \\	 &   5.11 &   4.82 &   3.5 &   6.74 &   5.63 &   4.11 \\
RAVE J050600.7-351056 & 	 +0.02$\pm$0.14 [16]  & 	  $-$0.37$\pm$0.10 [2]  & 	 +0.19$\pm$0.2 [1]  & 	  $-$1.98$\pm$0.14 [93]  & 	  $-$0.03$\pm$0.13 [8]  & 	 +0.20$\pm$0.10 [2]  \\	 &   3.68 &   3.08 &   3.2 &   5.52 &   4.21 &   2.78 \\
RAVE J050947.6-442317 & 	  $-$0.20$\pm$0.08 [6]  & 	  $-$0.17$\pm$0.12 [4]  & 	 ...  & 	  $-$2.50$\pm$0.10 [83]  & 	 +0.17$\pm$0.23 [3]  & 	 +0.34$\pm$0.10 [2]  \\	 &   2.94 &   2.76 &  ... &   5.00 &   3.89 &   2.40 \\
RAVE J053817.0-751621 & 	  $-$0.16$\pm$0.13 [22]  & 	  $-$0.57$\pm$0.32 [5]  & 	  $-$0.46$\pm$0.1 [2]  & 	  $-$2.03$\pm$0.14 [132]  & 	 +0.00$\pm$0.10 [15]  & 	  $-$0.03$\pm$0.10 [2]  \\	 &   3.45 &   2.83 &   2.63 &   5.47 &   4.19 &   2.50 \\
2MASS J05510847-5523127 & 	  $-$0.10$\pm$0.15 [19]  & 	  $-$0.37$\pm$0.20 [1]  & 	 +0.23$\pm$0.2 [1]  & 	  $-$2.31$\pm$0.10 [92]  & 	 +0.04$\pm$0.14 [14]  & 	 +0.15$\pm$0.10 [2]  \\	 &   3.23 &   2.75 &   2.91 &   5.19 &   3.95 &   2.40 \\
RAVE J061950.0-531212 & 	  $-$0.12$\pm$0.17 [22]  & 	  $-$0.28$\pm$0.25 [3]  & 	 +0.46$\pm$0.19 [5]  & 	  $-$2.09$\pm$0.16 [135]  & 	 +0.08$\pm$0.10 [16]  & 	 +0.48$\pm$0.10 [2]  \\	 &   3.43 &   3.06 &   3.36 &   5.41 &   4.21 &   2.95 \\
2MASS J06340181-4707492 & 	  $-$0.09$\pm$0.11 [14]  & 	  $-$0.28$\pm$0.25 [4]  & 	 +0.22$\pm$0.19 [2]  & 	  $-$2.26$\pm$0.10 [97]  & 	 +0.06$\pm$0.12 [11]  & 	 +0.21$\pm$0.10 [2]  \\	 &   3.29 &   2.89 &   2.95 &   5.24 &   4.02 &   2.51 \\
RAVE J063736.3-692947 & 	  $-$0.25$\pm$0.14 [9]  & 	  $-$0.05$\pm$0.20 [1]  & 	 ...  & 	  $-$1.67$\pm$0.24 [72]  & 	  $-$0.10$\pm$0.25 [4]  & 	 ...  \\	 &   3.72 &   3.71 &  ... &   5.83 &   4.45 &  ....00 \\
RAVE J070520.3-334324 & 	  $-$0.09$\pm$0.17 [19]  & 	  $-$0.33$\pm$0.10 [2]  & 	 +0.16$\pm$0.25 [2]  & 	  $-$2.43$\pm$0.13 [127]  & 	 +0.07$\pm$0.11 [12]  & 	 +0.14$\pm$0.10 [2]  \\	 &   3.12 &   2.67 &   2.72 &   5.07 &   3.86 &   2.27 \\
RAVE J074824.3-483141 & 	  $-$0.03$\pm$0.14 [22]  & 	  $-$0.08$\pm$0.29 [7]  & 	 +0.14$\pm$0.15 [4]  & 	  $-$2.01$\pm$0.11 [133]  & 	 +0.05$\pm$0.10 [16]  & 	 +0.12$\pm$0.10 [2]  \\	 &   3.6 &   3.34 &   3.12 &   5.49 &   4.26 &   2.67 \\
RAVE J100709.2-180947 & 	  $-$0.08$\pm$0.29 [21]  & 	  $-$0.40$\pm$0.12 [2]  & 	 ...  & 	  $-$1.92$\pm$0.15 [102]  & 	 +0.04$\pm$0.15 [10]  & 	 +0.13$\pm$0.10 [2]  \\	 &   3.64 &   3.11 &  ... &   5.58 &   4.34 &   2.77 \\
RAVE J100824.9-231412 & 	  $-$0.08$\pm$0.14 [9]  & 	  $-$0.40$\pm$0.10 [2]  & 	 ...  & 	  $-$1.95$\pm$0.13 [88]  & 	  $-$0.05$\pm$0.19 [8]  & 	  $-$0.04$\pm$0.20 [1]  \\	 &   3.61 &   3.08 &  ... &   5.55 &   4.22 &   2.57 \\
RAVE J101621.6-295952 & 	  $-$0.10$\pm$0.13 [21]  & 	 +0.03$\pm$0.41 [7]  & 	 +0.49$\pm$0.22 [5]  & 	  $-$2.12$\pm$0.12 [113]  & 	  $-$0.01$\pm$0.10 [15]  & 	 +0.11$\pm$0.10 [2]  \\	 &   3.42 &   3.34 &   3.36 &   5.38 &   4.09 &   2.55 \\
RAVE J112651.4-180530 & 	  $-$0.21$\pm$0.18 [11]  & 	 +0.02$\pm$0.51 [3]  & 	 +0.62$\pm$0.2 [1]  & 	  $-$2.52$\pm$0.13 [93]  & 	  $-$0.02$\pm$0.22 [6]  & 	 +0.06$\pm$0.16 [2]  \\	 &   2.91 &   2.93 &   3.09 &   4.98 &   3.68 &   2.10 \\
RAVE J113508.3-111328 & 	 +0.01$\pm$0.16 [21]  & 	 +0.00$\pm$0.26 [6]  & 	 +0.43$\pm$0.13 [3]  & 	  $-$1.32$\pm$0.12 [98]  & 	  $-$0.06$\pm$0.17 [14]  & 	 +0.07$\pm$0.10 [2]  \\	 &   4.33 &   4.11 &   4.1 &   6.18 &   4.84 &   3.31 \\
RAVE J114444.8-112817 & 	  $-$0.12$\pm$0.08 [22]  & 	  $-$0.25$\pm$0.17 [7]  & 	 +0.04$\pm$0.11 [4]  & 	  $-$2.63$\pm$0.08 [126]  & 	 +0.09$\pm$0.12 [15]  & 	 +0.26$\pm$0.10 [2]  \\	 &   2.89 &   2.55 &   2.4 &   4.87 &   3.68 &   2.19 \\
RAVE J115337.3-020037 & 	  $-$0.11$\pm$0.31 [8]  & 	  $-$0.61$\pm$0.22 [2]  & 	  $-$0.03$\pm$0.2 [1]  & 	  $-$2.43$\pm$0.12 [81]  & 	 +0.10$\pm$0.10 [7]  & 	 +0.38$\pm$0.20 [2]  \\	 &   3.1 &   2.39 &   2.53 &   5.07 &   3.89 &   2.51 \\
RAVE J115941.7-382043 & 	 +0.06$\pm$0.16 [24]  & 	 +0.34$\pm$0.10 [3]  & 	 +0.86$\pm$0.32 [4]  & 	  $-$1.23$\pm$0.10 [104]  & 	 +0.13$\pm$0.14 [16]  & 	 +0.34$\pm$0.10 [2]  \\	 &   4.47 &   4.54 &   4.62 &   6.27 &   5.12 &   3.67 \\
RAVE J123550.1-313111 & 	  $-$0.06$\pm$0.19 [19]  & 	  $-$0.29$\pm$0.10 [3]  & 	 +0.75$\pm$0.4 [3]  & 	  $-$2.59$\pm$0.13 [91]  & 	 +0.17$\pm$0.17 [12]  & 	 +0.18$\pm$0.10 [2]  \\	 &   2.99 &   2.55 &   3.15 &   4.91 &   3.80 &   2.15 \\
RAVE J115941.7-382043 & 	  $-$0.10$\pm$0.27 [7]  & 	  $-$0.28$\pm$0.20 [1]  & 	 ...  & 	  $-$2.27$\pm$0.16 [69]  & 	 +0.10$\pm$0.12 [4]  & 	 ...  \\	 &   3.27 &   2.88 &   3.59 &   5.23 &   4.05 &  ....00 \\
RAVE J124718.3-555047 & 	 +0.08$\pm$0.34 [16]  & 	  $-$0.30$\pm$0.10 [2]  & 	 ...  & 	  $-$2.00$\pm$0.13 [79]  & 	 +0.07$\pm$0.15 [12]  & 	 +0.62$\pm$0.20 [1]  \\	 &   3.72 &   3.13 &  ... &   5.50 &   4.29 &   3.18 \\
RAVE J124753.3-390802 & 	  $-$0.09$\pm$0.13 [18]  & 	  $-$0.27$\pm$0.10 [3]  & 	 ...  & 	  $-$2.17$\pm$0.11 [61]  & 	  $-$0.01$\pm$0.16 [14]  & 	 +0.01$\pm$0.10 [2]  \\	 &   3.38 &   2.99 &  ... &   5.33 &   4.04 &   2.40 \\
RAVE J125728.3-512522 & 	  $-$0.21$\pm$0.22 [17]  & 	  $-$0.35$\pm$0.10 [4]  & 	 +0.86$\pm$0.2 [1]  & 	  $-$2.47$\pm$0.11 [103]  & 	 +0.01$\pm$0.10 [14]  & 	 +0.23$\pm$0.10 [2]  \\	 &   2.96 &   2.61 &   3.38 &   5.03 &   3.76 &   2.32 \\
RAVE J125807.3-450627 & 	 +0.05$\pm$0.20 [16]  & 	  $-$0.33$\pm$0.10 [3]  & 	 +0.83$\pm$0.2 [1]  & 	  $-$2.07$\pm$0.16 [69]  & 	  $-$0.07$\pm$0.17 [12]  & 	 +0.01$\pm$0.10 [2]  \\	 &   3.62 &   3.03 &   3.75 &   5.43 &   4.08 &   2.50 \\
RAVE J130231.2-144805 & 	  $-$0.03$\pm$0.07 [19]  & 	 +0.04$\pm$0.36 [5]  & 	 +0.13$\pm$0.1 [2]  & 	  $-$1.75$\pm$0.08 [102]  & 	 +0.05$\pm$0.10 [12]  & 	 +0.24$\pm$0.10 [2]  \\	 &   3.86 &   3.72 &   3.37 &   5.75 &   4.52 &   3.05 \\
RAVE J130404.1-240837 & 	  $-$0.09$\pm$0.11 [19]  & 	 +0.00$\pm$0.14 [4]  & 	 +0.29$\pm$0.25 [4]  & 	  $-$2.17$\pm$0.12 [117]  & 	 +0.08$\pm$0.10 [15]  & 	 +0.45$\pm$0.10 [2]  \\	 &   3.38 &   3.26 &   3.11 &   5.33 &   4.13 &   2.84 \\
RAVE J130455.0-371249 & 	 +0.03$\pm$0.16 [14]  & 	 +0.27$\pm$0.27 [4]  & 	 +0.47$\pm$0.1 [2]  & 	  $-$0.89$\pm$0.08 [74]  & 	 +0.11$\pm$0.16 [13]  & 	  $-$0.01$\pm$0.10 [2]  \\	 &   4.78 &   4.81 &   4.57 &   6.61 &   5.44 &   3.66 \\
RAVE J133352.8-262354 & 	  $-$0.07$\pm$0.09 [21]  & 	  $-$0.17$\pm$0.23 [4]  & 	 +0.51$\pm$0.23 [5]  & 	  $-$2.27$\pm$0.09 [115]  & 	 +0.04$\pm$0.11 [14]  & 	 +0.26$\pm$0.10 [2]  \\	 &   3.3 &   2.99 &   3.23 &   5.23 &   3.99 &   2.55 \\
RAVE J134723.7-314409 & 	  $-$0.12$\pm$0.08 [18]  & 	  $-$0.35$\pm$0.19 [4]  & 	 ...  & 	  $-$1.99$\pm$0.11 [126]  & 	  $-$0.08$\pm$0.10 [13]  & 	  $-$0.01$\pm$0.10 [2]  \\	 &   3.53 &   3.09 &  ... &   5.51 &   4.15 &   2.56 \\
RAVE J135735.4-303249 & 	  $-$0.08$\pm$0.20 [15]  & 	  $-$0.20$\pm$0.30 [5]  & 	 ...  & 	  $-$2.46$\pm$0.10 [118]  & 	 +0.04$\pm$0.15 [10]  & 	 +0.43$\pm$0.12 [2]  \\	 &   3.1 &   2.77 &  ... &   5.04 &   3.80 &   2.53 \\
RAVE J140329.0-525043 & 	  $-$0.08$\pm$0.10 [14]  & 	  $-$0.40$\pm$0.20 [1]  & 	 +0.57$\pm$0.2 [1]  & 	  $-$1.93$\pm$0.10 [92]  & 	 +0.02$\pm$0.11 [14]  & 	 +0.10$\pm$0.10 [2]  \\	 &   3.63 &   3.1 &   3.63 &   5.57 &   4.31 &   2.73 \\
RAVE J140335.4-333526 & 	  $-$0.04$\pm$0.25 [6]  & 	  $-$0.40$\pm$0.10 [2]  & 	 +0.44$\pm$0.2 [1]  & 	  $-$2.75$\pm$0.10 [78]  & 	 +0.11$\pm$0.21 [5]  & 	 +0.18$\pm$0.20 [1]  \\	 &   2.85 &   2.28 &   2.68 &   4.75 &   3.58 &   1.99 \\
RAVE J141126.2-113746 & 	  $-$0.20$\pm$0.25 [11]  & 	  $-$0.38$\pm$0.20 [1]  & 	 ...  & 	  $-$2.75$\pm$0.12 [64]  & 	 +0.23$\pm$0.11 [9]  & 	 +0.51$\pm$0.10 [2]  \\	 &   2.69 &   2.3 &  ... &   4.75 &   3.70 &   2.32 \\
RAVE J141253.2-355256 & 	  $-$0.18$\pm$0.11 [19]  & 	  $-$0.17$\pm$0.33 [5]  & 	 +0.5$\pm$0.23 [2]  & 	  $-$2.45$\pm$0.08 [94]  & 	 +0.02$\pm$0.15 [12]  & 	 +0.07$\pm$0.20 [1]  \\	 &   3.01 &   2.81 &   3.04 &   5.05 &   3.79 &   2.18 \\
RAVE J153830.9-180424 & 	  $-$0.09$\pm$0.24 [25]  & 	  $-$0.13$\pm$0.32 [7]  & 	 +0.65$\pm$0.26 [5]  & 	  $-$2.20$\pm$0.11 [109]  & 	 +0.01$\pm$0.10 [16]  & 	 +0.12$\pm$0.10 [2]  \\	 &   3.35 &   3.1 &   3.44 &   5.30 &   4.03 &   2.48 \\
RAVE J155211.1-143037 & 	  $-$0.04$\pm$0.09 [19]  & 	  $-$0.07$\pm$0.36 [7]  & 	 +0.15$\pm$0.3 [5]  & 	  $-$1.60$\pm$0.12 [128]  & 	 +0.01$\pm$0.15 [16]  & 	 +0.06$\pm$0.10 [2]  \\	 &   4 &   3.76 &   3.54 &   5.90 &   4.63 &   3.02 \\
RAVE J155829.6-122434 & 	  $-$0.13$\pm$0.14 [18]  & 	  $-$0.23$\pm$0.26 [7]  & 	 +0.55$\pm$0.31 [5]  & 	  $-$2.82$\pm$0.09 [96]  & 	 +0.08$\pm$0.13 [13]  & 	 +0.43$\pm$0.10 [2]  \\	 &   2.69 &   2.38 &   2.72 &   4.68 &   3.48 &   2.17 \\
RAVE J160245.0-152102 & 	  $-$0.08$\pm$0.08 [25]  & 	  $-$0.13$\pm$0.28 [7]  & 	 +0.19$\pm$0.18 [3]  & 	  $-$2.05$\pm$0.10 [151]  & 	 +0.03$\pm$0.10 [16]  & 	 +0.20$\pm$0.10 [2]  \\	 &   3.51 &   3.25 &   3.13 &   5.45 &   4.20 &   2.71 \\
RAVE J161847.0-014540 & 	  $-$0.13$\pm$0.08 [20]  & 	  $-$0.46$\pm$0.10 [3]  & 	 ...  & 	  $-$2.09$\pm$0.10 [112]  & 	  $-$0.03$\pm$0.10 [11]  & 	 +0.19$\pm$0.10 [2]  \\	 &   3.42 &   2.88 &  ... &   5.41 &   4.10 &   2.66 \\
RAVE J161943.1-022431 & 	  $-$0.05$\pm$0.09 [14]  & 	  $-$0.40$\pm$0.10 [3]  & 	 +1$\pm$0.5 [2]  & 	  $-$2.24$\pm$0.09 [96]  & 	 +0.03$\pm$0.10 [12]  & 	 +0.19$\pm$0.10 [2]  \\	 &   3.35 &   2.79 &   3.75 &   5.26 &   4.01 &   2.51 \\
RAVE J165300.5-005507 & 	  $-$0.05$\pm$0.28 [24]  & 	 +0.03$\pm$0.41 [6]  & 	 +0.64$\pm$0.31 [4]  & 	  $-$1.63$\pm$0.13 [86]  & 	  $-$0.03$\pm$0.13 [14]  & 	 +0.07$\pm$0.10 [2]  \\	 &   3.96 &   3.83 &   4 &   5.87 &   4.56 &   3.00 \\
2MASS J17163340-7009028 & 	  $-$0.11$\pm$0.23 [12]  & 	  $-$0.22$\pm$0.20 [1]  & 	 ...  & 	  $-$2.69$\pm$0.15 [90]  & 	 +0.14$\pm$0.14 [9]  & 	 +0.37$\pm$0.10 [2]  \\	 &   2.84 &   2.52 &  ... &   4.81 &   3.67 &   2.24 \\
RAVE J175159.8-475131 & 	  $-$0.13$\pm$0.13 [17]  & 	  $-$0.39$\pm$0.10 [2]  & 	 +0.13$\pm$0.2 [1]  & 	  $-$2.20$\pm$0.11 [76]  & 	  $-$0.06$\pm$0.14 [16]  & 	 +0.14$\pm$0.10 [2]  \\	 &   3.31 &   2.84 &   2.92 &   5.30 &   3.96 &   2.50 \\
RAVE J180242.3-440443 & 	  $-$0.06$\pm$0.13 [13]  & 	  $-$0.06$\pm$0.16 [3]  & 	 ...  & 	  $-$1.88$\pm$0.12 [104]  & 	  $-$0.05$\pm$0.11 [10]  & 	 +0.13$\pm$0.10 [2]  \\	 &   3.7 &   3.49 &  ... &   5.62 &   4.29 &   2.81 \\
RAVE J183108.2-491105 & 	  $-$0.17$\pm$0.25 [20]  & 	  $-$0.40$\pm$0.10 [3]  & 	  $-$0.19$\pm$0.2 [1]  & 	  $-$2.08$\pm$0.18 [118]  & 	  $-$0.06$\pm$0.11 [15]  & 	 +0.02$\pm$0.10 [2]  \\	 &   3.39 &   2.95 &   2.72 &   5.42 &   4.08 &   2.50 \\
RAVE J183623.2-642812 & 	  $-$0.18$\pm$0.19 [7]  & 	 ...  & 	 +0.5$\pm$0.2 [1]  & 	  $-$2.54$\pm$0.08 [71]  & 	 +0.07$\pm$0.10 [5]  & 	 +0.23$\pm$0.12 [2]  \\	 &   2.92 &  ... &   2.95 &   4.96 &   3.75 &   2.25 \\
2MASS J19031845-5138510 & 	  $-$0.16$\pm$0.23 [9]  & 	  $-$0.39$\pm$0.20 [1]  & 	 ...  & 	  $-$2.15$\pm$0.16 [89]  & 	 +0.00$\pm$0.10 [6]  & 	 +0.11$\pm$0.20 [1]  \\	 &   3.33 &   2.89 &  ... &   5.35 &   4.07 &   2.52 \\
RAVE J190733.1-415832 & 	  $-$0.19$\pm$0.14 [14]  & 	  $-$0.40$\pm$0.10 [3]  & 	 +0.66$\pm$0.2 [1]  & 	  $-$2.44$\pm$0.13 [81]  & 	 +0.02$\pm$0.10 [12]  & 	 +0.28$\pm$0.11 [2]  \\	 &   3.01 &   2.59 &   3.21 &   5.06 &   3.80 &   2.40 \\
RAVE J190923.1-435357 & 	  $-$0.24$\pm$0.18 [11]  & 	  $-$0.33$\pm$0.10 [3]  & 	 ...  & 	  $-$2.05$\pm$0.14 [98]  & 	 +0.03$\pm$0.11 [11]  & 	  $-$0.06$\pm$0.20 [1]  \\	 &   3.35 &   3.05 &  ... &   5.45 &   4.20 &   2.45 \\
RAVE J191755.9-544015 & 	  $-$0.12$\pm$0.18 [23]  & 	  $-$0.09$\pm$0.22 [7]  & 	 +0.45$\pm$0.13 [5]  & 	  $-$2.81$\pm$0.10 [131]  & 	 +0.19$\pm$0.10 [14]  & 	 +0.21$\pm$0.10 [2]  \\	 &   2.71 &   2.53 &   2.63 &   4.69 &   3.60 &   1.96 \\
RAVE J192325.2-583341 & 	  $-$0.10$\pm$0.16 [15]  & 	  $-$0.20$\pm$0.25 [4]  & 	 ...  & 	  $-$2.41$\pm$0.13 [111]  & 	 +0.06$\pm$0.10 [9]  & 	 +0.34$\pm$0.10 [2]  \\	 &   3.13 &   2.82 &  ... &   5.09 &   3.87 &   2.49 \\
RAVE J192819.9-633935 & 	  $-$0.14$\pm$0.14 [21]  & 	  $-$0.22$\pm$0.25 [7]  & 	 +0.09$\pm$0.14 [3]  & 	  $-$2.40$\pm$0.11 [130]  & 	 +0.01$\pm$0.10 [15]  & 	 +0.17$\pm$0.10 [2]  \\	 &   3.1 &   2.81 &   2.49 &   5.10 &   3.83 &   2.33 \\
RAVE J193102.8-440158 & 	  $-$0.16$\pm$0.10 [20]  & 	  $-$0.26$\pm$0.33 [6]  & 	 +0.22$\pm$0.16 [3]  & 	  $-$2.28$\pm$0.13 [121]  & 	  $-$0.01$\pm$0.10 [15]  & 	 +0.15$\pm$0.10 [2]  \\	 &   3.2 &   2.89 &   2.93 &   5.22 &   3.93 &   2.43 \\
RAVE J194318.7-594820 & 	  $-$0.28$\pm$0.11 [17]  & 	 +0.12$\pm$0.37 [5]  & 	 ...  & 	  $-$2.17$\pm$0.13 [89]  & 	  $-$0.13$\pm$0.15 [0.16]  & 	 +0.12$\pm$0.10 [2]  \\	 &   3.19 &   3.38 &  ... &   5.33 &   3.92 &   2.51 \\
RAVE J194319.0-405425 & 	  $-$0.03$\pm$0.11 [18]  & 	  $-$0.02$\pm$0.33 [6]  & 	 +0.1$\pm$0.2 [1]  & 	  $-$1.72$\pm$0.10 [137]  & 	  $-$0.03$\pm$0.14 [10]  & 	  $-$0.07$\pm$0.10 [2]  \\	 &   3.89 &   3.69 &   3.37 &   5.78 &   4.47 &   2.77 \\
RAVE J194550.6-392631 & 	  $-$0.19$\pm$0.19 [22]  & 	  $-$0.43$\pm$0.16 [7]  & 	 +0.41$\pm$0.1 [4]  & 	  $-$2.97$\pm$0.09 [116]  & 	 +0.12$\pm$0.15 [13]  & 	 +0.23$\pm$0.10 [2]  \\	 &   2.48 &   2.03 &   2.43 &   4.53 &   3.37 &   1.82 \\
RAVE J200034.7-342004 & 	  $-$0.18$\pm$0.09 [18]  & 	  $-$0.30$\pm$0.10 [2]  & 	 ...  & 	  $-$2.12$\pm$0.14 [116]  & 	 +0.03$\pm$0.10 [11]  & 	 +0.32$\pm$0.20 [1]  \\	 &   3.34 &   3.01 &  ... &   5.38 &   4.13 &   2.76 \\
RAVE J200057.7-254149 & 	  $-$0.13$\pm$0.09 [18]  & 	  $-$0.03$\pm$0.54 [4]  & 	 +0.53$\pm$0.1 [3]  & 	  $-$2.09$\pm$0.11 [107]  & 	 +0.02$\pm$0.10 [13]  & 	 +0.16$\pm$0.10 [2]  \\	 &   3.42 &   3.31 &   3.43 &   5.41 &   4.15 &   2.63 \\
RAVE J201007.1-515502 & 	  $-$0.20$\pm$0.22 [21]  & 	  $-$0.84$\pm$0.47 [4]  & 	  $-$0.3$\pm$0.2 [1]  & 	  $-$2.56$\pm$0.12 [100]  & 	 +0.03$\pm$0.10 [13]  & 	 +0.15$\pm$0.10 [2]  \\	 &   2.88 &   2.03 &   2.13 &   4.94 &   3.69 &   2.15 \\
RAVE J202029.2-270735 & 	  $-$0.13$\pm$0.13 [8]  & 	  $-$0.73$\pm$0.24 [2]  & 	 +0.68$\pm$0.2 [1]  & 	  $-$3.01$\pm$0.11 [83]  & 	 +0.07$\pm$0.10 [3]  & 	 +0.36$\pm$0.13 [2]  \\	 &   2.5 &   1.69 &   2.66 &   4.49 &   3.28 &   1.91 \\
RAVE J202432.1-151029 & 	  $-$0.08$\pm$0.15 [17]  & 	  $-$0.07$\pm$0.10 [3]  & 	 +0.41$\pm$0.27 [2]  & 	  $-$1.71$\pm$0.12 [94]  & 	 +0.03$\pm$0.12 [14]  & 	 +0.15$\pm$0.10 [2]  \\	 &   3.85 &   3.65 &   3.96 &   5.79 &   4.54 &   3.00 \\
RAVE J202434.5-423334 & 	  $-$0.39$\pm$0.24 [9]  & 	  $-$0.30$\pm$0.17 [2]  & 	 +0.21$\pm$0.2 [1]  & 	  $-$2.68$\pm$0.17 [88]  & 	 +0.22$\pm$0.36 [6]  & 	 +0.14$\pm$0.17 [2]  \\	 &   2.57 &   2.45 &   2.52 &   4.82 &   3.76 &   2.02 \\
2MASS J20264253-1656467 & 	  $-$0.13$\pm$0.11 [20]  & 	  $-$0.15$\pm$0.22 [5]  & 	 +0.13$\pm$0.2 [1]  & 	  $-$1.97$\pm$0.16 [121]  & 	  $-$0.02$\pm$0.10 [17]  & 	 +0.00$\pm$0.20 [1]  \\	 &   3.54 &   3.31 &   3.15 &   5.53 &   4.23 &   2.59 \\
RAVE J202654.7-595013 & 	  $-$0.11$\pm$0.07 [17]  & 	  $-$0.02$\pm$0.47 [6]  & 	 +0.34$\pm$0.11 [4]  & 	  $-$2.05$\pm$0.11 [122]  & 	  $-$0.01$\pm$0.11 [13]  & 	 +0.23$\pm$0.10 [2]  \\	 &   3.48 &   3.36 &   3.28 &   5.45 &   4.16 &   2.74 \\
RAVE J203428.4-241830 & 	  $-$0.18$\pm$0.13 [18]  & 	  $-$0.25$\pm$0.49 [7]  & 	 +0.64$\pm$0.15 [3]  & 	  $-$2.48$\pm$0.12 [128]  & 	 +0.01$\pm$0.17 [12]  & 	 +0.01$\pm$0.20 [1]  \\	 &   2.98 &   2.7 &   3.15 &   5.02 &   3.75 &   2.09 \\
RAVE J203622.6-071420 & 	  $-$0.04$\pm$0.09 [14]  & 	  $-$0.23$\pm$0.10 [3]  & 	 ...  & 	  $-$2.59$\pm$0.11 [36]  & 	 +0.09$\pm$0.14 [7]  & 	 +0.10$\pm$0.12 [2]  \\	 &   3.01 &   2.61 &  ... &   4.91 &   3.72 &   2.07 \\
RAVE J203706.4-122125 & 	  $-$0.21$\pm$0.13 [15]  & 	  $-$0.33$\pm$0.10 [3]  & 	 +0.31$\pm$0.23 [5]  & 	  $-$2.61$\pm$0.14 [85]  & 	 +0.02$\pm$0.12 [13]  & 	 +0.08$\pm$0.20 [1]  \\	 &   2.82 &   2.49 &   2.69 &   4.89 &   3.63 &   2.03 \\
RAVE J204355.8-563629 & 	  $-$0.18$\pm$0.12 [17]  & 	  $-$0.40$\pm$0.16 [4]  & 	 +0.24$\pm$0.19 [2]  & 	  $-$2.07$\pm$0.11 [136]  & 	  $-$0.05$\pm$0.10 [15]  & 	 +0.06$\pm$0.10 [2]  \\	 &   3.39 &   2.96 &   3.16 &   5.43 &   4.10 &   2.55 \\
RAVE J204450.7-371400 & 	  $-$0.18$\pm$0.21 [4]  & 	  $-$0.17$\pm$0.20 [1]  & 	 +0.09$\pm$0.2 [3]  & 	  $-$2.72$\pm$0.11 [64]  & 	 +0.23$\pm$0.12 [9]  & 	 +0.32$\pm$0.10 [2]  \\	 &   2.74 &   2.54 &   2.36 &   4.78 &   3.73 &   2.16 \\
RAVE J204954.4-480045 & 	  $-$0.12$\pm$0.08 [17]  & 	  $-$0.02$\pm$0.36 [7]  & 	 +0.42$\pm$0.37 [5]  & 	  $-$1.82$\pm$0.13 [152]  & 	  $-$0.09$\pm$0.10 [14]  & 	  $-$0.01$\pm$0.20 [2]  \\	 &   3.7 &   3.59 &   3.59 &   5.68 &   4.31 &   2.73 \\
RAVE J205149.7-615801 & 	  $-$0.10$\pm$0.08 [24]  & 	  $-$0.07$\pm$0.22 [6]  & 	 +0.17$\pm$0.15 [4]  & 	  $-$2.03$\pm$0.11 [121]  & 	 +0.03$\pm$0.12 [15]  & 	 +0.19$\pm$0.10 [2]  \\	 &   3.51 &   3.33 &   3.13 &   5.47 &   4.22 &   2.72 \\
RAVE J205609.1-133118 & 	  $-$0.15$\pm$0.15 [25]  & 	  $-$0.24$\pm$0.28 [7]  & 	 +0.29$\pm$0.23 [5]  & 	  $-$2.33$\pm$0.10 [140]  & 	  $-$0.01$\pm$0.10 [16]  & 	 +0.09$\pm$0.10 [2]  \\	 &   3.16 &   2.86 &   2.95 &   5.17 &   3.88 &   2.32 \\
RAVE J210634.7-495750 & 	  $-$0.29$\pm$0.14 [8]  & 	  $-$0.45$\pm$0.10 [4]  & 	 +0.35$\pm$0.14 [4]  & 	  $-$3.24$\pm$0.06 [91]  & 	 +0.22$\pm$0.10 [4]  & 	 +0.34$\pm$0.10 [2]  \\	 &   2.11 &   1.74 &   2.1 &   4.26 &   3.20 &   1.66 \\
RAVE J210642.9-682827 & 	  $-$0.21$\pm$0.32 [13]  & 	  $-$0.35$\pm$0.16 [6]  & 	 +0.26$\pm$0.21 [5]  & 	  $-$2.95$\pm$0.12 [101]  & 	 +0.13$\pm$0.17 [9]  & 	 +0.42$\pm$0.10 [2]  \\	 &   2.48 &   2.13 &   2.3 &   4.55 &   3.40 &   2.03 \\
RAVE J211525.5-150331 & 	  $-$0.13$\pm$0.20 [10]  & 	  $-$0.38$\pm$0.20 [1]  & 	 ...  & 	  $-$2.08$\pm$0.22 [121]  & 	  $-$0.04$\pm$0.11 [9]  & 	 +0.17$\pm$0.12 [2]  \\	 &   3.43 &   2.97 &  ... &   5.42 &   4.10 &   2.65 \\
RAVE J211927.1-402908 & 	  $-$0.14$\pm$0.09 [19]  & 	  $-$0.22$\pm$0.14 [7]  & 	 +0.33$\pm$0.59 [3]  & 	  $-$2.15$\pm$0.12 [134]  & 	 +0.01$\pm$0.10 [15]  & 	 +0.15$\pm$0.10 [2]  \\	 &   3.35 &   3.06 &   3.17 &   5.35 &   4.08 &   2.56 \\
RAVE J212921.0-620915 & 	  $-$0.14$\pm$0.06 [15]  & 	  $-$0.18$\pm$0.22 [6]  & 	 +0.28$\pm$0.37 [2]  & 	  $-$2.46$\pm$0.09 [124]  & 	 +0.12$\pm$0.10 [11]  & 	 +0.30$\pm$0.20 [1]  \\	 &   3.04 &   2.79 &   2.81 &   5.04 &   3.88 &   2.40 \\ &  ...
RAVE J215118.3-135937 & 	  $-$0.06$\pm$0.29 [9]  & 	  $-$0.45$\pm$0.16 [2]  & 	  $-$0.39$\pm$0.2 [1]  & 	  $-$1.99$\pm$0.16 [90]  & 	  $-$0.02$\pm$0.11 [5]  & 	 +0.14$\pm$0.12 [2]  \\	 &   3.59 &   2.99 &   2.61 &   5.51 &   4.21 &   2.71 \\
RAVE J220211.8-441702 & 	  $-$0.12$\pm$0.16 [12]  & 	  $-$0.24$\pm$0.10 [4]  & 	 +0.34$\pm$0.11 [3]  & 	  $-$2.88$\pm$0.09 [103]  & 	 +0.16$\pm$0.10 [5]  & 	 +0.35$\pm$0.20 [1]  \\	 &   2.64 &   2.31 &   2.45 &   4.62 &   3.50 &   2.03 \\
RAVE J220403.6-402919 & 	  $-$0.21$\pm$0.16 [6]  & 	  $-$0.37$\pm$0.20 [1]  & 	 ...  & 	  $-$2.57$\pm$0.16 [86]  & 	 +0.07$\pm$0.11 [4]  & 	 +0.05$\pm$0.20 [1]  \\	 &   2.86 &   2.49 &   4.93 &   3.72 &   2.04 \\
2MASS J22122728-6810067 & 	  $-$0.04$\pm$0.10 [16]  & 	  $-$0.32$\pm$0.25 [3]  & 	 ...  & 	  $-$1.76$\pm$0.12 [97]  & 	 +0.03$\pm$0.20 [10]  & 	 +0.09$\pm$0.17 [2]  \\	 &   3.84 &   3.35 &  ... &   5.74 &   4.49 &   2.89 \\
RAVE J222236.0-013827 & 	  $-$0.17$\pm$0.24 [10]  & 	  $-$0.01$\pm$0.10 [2]  & 	 +0.91$\pm$0.2 [1]  & 	  $-$2.82$\pm$0.14 [85]  & 	 +0.19$\pm$0.16 [7]  & 	 +0.48$\pm$0.20 [1]  \\	 &   2.65 &   2.6 &   3.08 &   4.68 &   3.59 &   2.22 \\
RAVE J223716.2-160801 & 	 +0.08$\pm$0.23 [15]  & 	  $-$0.23$\pm$0.23 [5]  & 	 +0.29$\pm$0.24 [2]  & 	  $-$2.21$\pm$0.10 [91]  & 	 +0.24$\pm$0.27 [10]  & 	 +0.15$\pm$1.00 [0]  \\	 &   3.51 &   2.99 &   3.07 &   5.29 &   4.25 &   2.50 \\
RAVE J224927.6-223829 & 	  $-$0.05$\pm$0.23 [15]  & 	  $-$0.03$\pm$0.19 [4]  & 	  $-$0.37$\pm$0.2 [1]  & 	  $-$2.03$\pm$0.13 [77]  & 	  $-$0.04$\pm$0.14 [10]  & 	  $-$0.01$\pm$0.10 [2]  \\	 &   3.56 &   3.37 &   3.31 &   5.47 &   4.15 &   2.52 \\
RAVE J225319.9-224856 & 	  $-$0.17$\pm$0.08 [14]  & 	 +0.04$\pm$0.47 [3]  & 	 +0.09$\pm$0.2 [1]  & 	  $-$2.16$\pm$0.14 [111]  & 	  $-$0.06$\pm$0.10 [10]  & 	 +0.38$\pm$0.18 [2]  \\	 &   3.31 &   3.31 &   3.61 &   5.34 &   4.00 &   2.78 \\
RAVE J225926.9-523733 & 	  $-$0.12$\pm$0.13 [24]  & 	 +0.13$\pm$0.71 [6]  & 	 +0.15$\pm$0.13 [5]  & 	  $-$2.20$\pm$0.11 [117]  & 	 +0.02$\pm$0.10 [16]  & 	 +0.05$\pm$0.10 [2]  \\	 &   3.32 &   3.36 &   2.94 &   5.30 &   4.04 &   2.41 \\
RAVE J230222.9-683323 & 	  $-$0.10$\pm$0.15 [14]  & 	  $-$0.25$\pm$0.10 [4]  & 	 +0.39$\pm$0.2 [1]  & 	  $-$2.26$\pm$0.15 [115]  & 	 +0.05$\pm$0.15 [8]  & 	 +0.23$\pm$0.10 [2]  \\	 &   3.28 &   2.92 &   3.12 &   5.24 &   4.01 &   2.53 \\
RAVE J231300.0-450707 & 	  $-$0.24$\pm$0.16 [11]  & 	  $-$0.46$\pm$0.11 [3]  & 	 +0.34$\pm$0.2 [1]  & 	  $-$2.53$\pm$0.12 [95]  & 	 +0.03$\pm$0.20 [1]  & 	 +0.24$\pm$0.20 [1]  \\	 &   2.87 &   2.44 &   2.8 &   4.97 &   3.72 &   2.27 \\
2MASS J23131638-7011223 & 	  $-$0.17$\pm$0.15 [21]  & 	  $-$0.52$\pm$0.20 [1]  & 	 +0.12$\pm$0.2 [1]  & 	  $-$2.19$\pm$0.09 [110]  & 	  $-$0.04$\pm$0.13 [14]  & 	 +0.12$\pm$0.10 [2]  \\	 &   3.28 &   2.72 &   2.92 &   5.31 &   3.99 &   2.49 \\
\enddata
\end{deluxetable*}

==> Table7_CandNCaptureAbundances.tex <==
\startlongtable

\begin{deluxetable*}{ccccccccc}
\tablecaption{\label{tab:ab3}Classifications, Carbon, and Neutron-capture Elements}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{NAME}  &
\colhead{Class}  &
\colhead{[C/Fe] (syn)} & 
\colhead{[C/Fe]$_{c}$} &
\colhead{$A$(C)$_{c}$} &
\colhead{[Sr/Fe]} & 
\colhead{[Ba/Fe] (syn)} & 
\colhead{[Eu/Fe] (syn)} &  
\colhead{[Ba/Eu]} \\
 &
 &
 &
 &
 &
 \colhead{log$\epsilon$(Sr)} &
 \colhead{log$\epsilon$(Ba)} &
 \colhead{log$\epsilon$(Eu)} &
}
\startdata
RAVE J000438.4-540134 & 	$r$-I & 	 +0.06$\pm$0.30 [1] & 	 +0.55$\pm$0.30 & 	6.60 & 	 +0.35$\pm$0.20 [1] &	 +0.16$\pm$0.20 [2]  &	 +0.61$\pm$0.20 [2 ] &	  $-$0.45$\pm$0.28 \\	 &  &  &  &  &   0.84 &  $-$0.04 &  $-$1.25 &  \\
RAVE J001236.5-181631 & 	... & 	  $-$0.01$\pm$0.30 [1] & 	 +0.00$\pm$0.30 & 	6.02 & 	  $-$0.14$\pm$0.10 [2] &	  $-$0.60$\pm$0.20 [2]  &	 +0.17$\pm$0.20 [2 ] &	  $-$0.76$\pm$0.28 \\	 &  &  &  &  &   0.32 &  $-$0.83 &  $-$1.72 &  \\
RAVE J003946.9-684957 & 	CEMP-no & 	 +0.10$\pm$0.30 [1] & 	 +0.73$\pm$0.30 & 	6.54 & 	 +0.43$\pm$0.20 [1] &	  $-$0.10$\pm$0.20 [1]  &	 +0.28$\pm$0.20 [3 ] &	  $-$0.38$\pm$0.28 \\	 &  &  &  &  &   0.68 &  $-$0.54 &  $-$1.82 &  \\
RAVE J010839.6-285701 & 	CEMP-$r$ & 	 +0.10$\pm$0.30 [1] & 	 +0.76$\pm$0.30 & 	6.32 & 	 +0.41$\pm$0.20 [1] &	  $-$0.52$\pm$0.20 [2]  &	 +0.45$\pm$0.20 [1 ] &	  $-$0.97$\pm$0.28 \\	 &  &  &  &  &   0.41 &  $-$1.21 &  $-$1.90 &  \\
2MASS J01162885-5343408 & 	... & 	  $-$0.02$\pm$0.30 [1] & 	 +0.39$\pm$0.30 & 	6.06 & 	  $-$0.19$\pm$0.20 [1] &	 +0.17$\pm$0.20 [1]  &	 ... &	 ... \\	 &  &  &  &  &  $-$0.08 &  $-$0.41 &  ... &  \\
2MASS J01201051-4849461 & 	... & 	  $-$0.12$\pm$0.30 [1] & 	 +0.20$\pm$0.30 & 	6.46 & 	 +0.03$\pm$0.20 [1] &	 +0.08$\pm$0.20 [2]  &	 +0.03$\pm$0.20 [1 ] &	 +0.06$\pm$0.28 \\	 &  &  &  &  &   0.73 &   0.09 &  $-$1.62 &  \\
RAVE J012931.1-160046 & 	CEMP-$r$ & 	 +0.26$\pm$0.30 [1] & 	 +0.95$\pm$0.30 & 	6.40 & 	 +0.45$\pm$0.20 [1] &	 +1.11$\pm$0.20 [2]  &	 +1.68$\pm$0.20 [3 ] &	  $-$0.57$\pm$0.28 \\	 &  &  &  &  &   0.34 &   0.31 &  $-$0.78 &  \\
RAVE J013807.0-195210 & 	$r$-I & 	  $-$0.09$\pm$0.30 [1] & 	  $-$0.08$\pm$0.30 & 	6.30 & 	 +0.05$\pm$0.20 [1] &	 +0.30$\pm$0.20 [2]  &	 +0.46$\pm$0.20 [1 ] &	  $-$0.16$\pm$0.28 \\	 &  &  &  &  &   0.87 &   0.43 &  $-$1.07 &  \\
RAVE J014254.2-503249 & 	$r$-I & 	 +0.25$\pm$0.30 [1] & 	 +0.26$\pm$0.30 & 	6.51 & 	 +0.08$\pm$0.20 [1] &	 +0.04$\pm$0.20 [2]  &	 +0.40$\pm$0.20 [2 ] &	  $-$0.36$\pm$0.28 \\	 &  &  &  &  &   0.77 &   0.04 &  $-$1.26 &  \\
RAVE J014908.0-491143 & 	CEMP-$r$ & 	 +0.07$\pm$0.30 [1] & 	 +0.81$\pm$0.30 & 	6.16 & 	  $-$0.01$\pm$0.20 [1] &	  $-$0.39$\pm$0.20 [2]  &	 +0.35$\pm$0.20 [3 ] &	  $-$0.74$\pm$0.28 \\	 &  &  &  &  &  $-$0.22 &  $-$1.29 &  $-$2.21 &  \\
RAVE J021110.2-191124 & 	$r$-I & 	 +0.05$\pm$0.30 [1] & 	 +0.06$\pm$0.30 & 	6.12 & 	  $-$0.04$\pm$0.20 [1] &	 +0.22$\pm$0.20 [2]  &	 +0.45$\pm$0.20 [1 ] &	  $-$0.23$\pm$0.28 \\	 &  &  &  &  &   0.46 &   0.03 &  $-$1.40 &  \\
RAVE J022013.3-601436 & 	$r$-I & 	  $-$0.06$\pm$0.30 [1] & 	 +0.17$\pm$0.30 & 	6.93 & 	 +0.12$\pm$0.20 [1] &	 +0.19$\pm$0.20 [2]  &	 +0.44$\pm$0.20 [2 ] &	  $-$0.25$\pm$0.28 \\	 &  &  &  &  &   1.32 &   0.70 &  $-$0.71 &  \\
RAVE J030639.1-692040 & 	CEMP-$r$ & 	 +0.10$\pm$0.30 [1] & 	 +0.79$\pm$0.30 & 	6.43 & 	  $-$0.02$\pm$0.20 [1] &	 +0.20$\pm$0.20 [2]  &	 +0.32$\pm$0.20 [3 ] &	  $-$0.12$\pm$0.28 \\	 &  &  &  &  &   0.06 &  $-$0.41 &  $-$1.95 &  \\
2MASS J03135637-6554095 & 	... & 	 +0.07$\pm$0.30 [1] & 	 +0.29$\pm$0.30 & 	6.29 & 	  $-$0.41$\pm$0.20 [1] &	  $-$0.82$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   0.03 &  $-$1.07 &  ... &  \\
RAVE J034228.2-650036 & 	$r$-II & 	 +0.06$\pm$0.30 [1] & 	 +0.46$\pm$0.30 & 	6.59 & 	 +0.38$\pm$0.20 [1] &	 +0.71$\pm$0.20 [2]  &	 +0.83$\pm$0.20 [3 ] &	  $-$0.12$\pm$0.28 \\	 &  &  &  &  &   0.95 &   0.59 &  $-$0.95 &  \\
2MASS J04042657-2229357 & 	... & 	 +0.09$\pm$0.30 [1] & 	 +0.10$\pm$0.30 & 	6.67 & 	 +0.13$\pm$0.20 [1] &	 +0.11$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   1.14 &   0.43 &  ... &  \\
RAVE J040658.7-540556 & 	... & 	 +0.34$\pm$0.30 [1] & 	 +0.35$\pm$0.30 & 	6.29 & 	 +0.28$\pm$0.20 [1] &	 +0.10$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   0.66 &  $-$0.21 &  ... &  \\
RAVE J045322.6-221040 & 	... & 	 +0.00$\pm$0.30 [1] & 	 ... & 	... & 	 +0.15$\pm$0.15 [2] &	  $-$0.58$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   0.71 &  $-$0.71 &  ... &  \\
2MASS J05023178-4540502 & 	... & 	  $-$1.15$\pm$0.30 [1] & 	  $-$1.15$\pm$0.30 & 	6.52 & 	 +0.11$\pm$0.20 [1] &	 +0.25$\pm$0.20 [1]  &	 ... &	 ... \\	 &  &  &  &  &   2.22 &   1.67 &  ... &  \\
RAVE J050600.7-351056 & 	$r$-I & 	 +0.01$\pm$0.30 [1] & 	 +0.01$\pm$0.30 & 	6.46 & 	  $-$0.12$\pm$0.10 [2] &	 +0.15$\pm$0.20 [2]  &	 +0.46$\pm$0.20 [1 ] &	  $-$0.31$\pm$0.28 \\	 &  &  &  &  &   0.77 &   0.35 &  $-$1.00 &  \\
RAVE J050947.6-442317 & 	... & 	 +0.52$\pm$0.30 [1] & 	 +0.52$\pm$0.30 & 	6.45 & 	 +0.33$\pm$0.10 [2] &	  $-$0.03$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   0.70 &  $-$0.35 &  ... &  \\
RAVE J053817.0-751621 & 	... & 	  $-$0.28$\pm$0.30 [1] & 	 +0.27$\pm$0.30 & 	6.67 & 	  $-$0.19$\pm$0.20 [1] &	 +0.03$\pm$0.20 [2]  &	 +0.01$\pm$0.20 [3 ] &	 +0.02$\pm$0.28 \\	 &  &  &  &  &   0.65 &   0.18 &  $-$1.50 &  \\
2MASS J05510847-5523127 & 	... & 	 +0.00$\pm$0.30 [1] & 	 +0.34$\pm$0.30 & 	6.46 & 	 +0.20$\pm$0.20 [1] &	 +0.33$\pm$0.20 [2]  &	 +0.15$\pm$0.20 [1 ] &	 +0.19$\pm$0.28 \\	 &  &  &  &  &   0.76 &   0.20 &  $-$1.64 &  \\
RAVE J061950.0-531212 & 	$r$-I & 	 +0.33$\pm$0.30 [1] & 	 +0.34$\pm$0.30 & 	6.68 & 	 ... &	 +0.16$\pm$0.20 [2]  &	 +0.63$\pm$0.20 [3 ] &	  $-$0.47$\pm$0.28 \\	 &  &  &  &  &  ... &   0.25 &  $-$0.94 &  \\
2MASS J06340181-4707492 & 	... & 	  $-$0.25$\pm$0.30 [1] & 	  $-$0.20$\pm$0.30 & 	5.97 & 	  $-$0.16$\pm$0.21 [2] &	 +0.19$\pm$0.20 [2]  &	 +0.05$\pm$0.20 [2 ] &	 +0.14$\pm$0.28 \\	 &  &  &  &  &   0.45 &   0.11 &  $-$1.69 &  \\
RAVE J063736.3-692947 & 	... & 	  $-$0.62$\pm$0.30 [1] & 	  $-$0.62$\pm$0.30 & 	6.14 & 	 +0.35$\pm$0.27 [2] &	 +0.04$\pm$0.20 [1]  &	 +0.12$\pm$0.20 [3 ] &	  $-$0.09$\pm$0.28 \\	 &  &  &  &  &   1.55 &   0.55 &  $-$1.03 &  \\
RAVE J070520.3-334324 & 	CEMP-$r$ & 	 +0.26$\pm$0.30 [1] & 	 +0.76$\pm$0.30 & 	6.76 & 	 +0.20$\pm$0.20 [0] &	 +0.40$\pm$0.20 [2]  &	 +0.68$\pm$0.20 [3 ] &	  $-$0.28$\pm$0.28 \\	 &  &  &  &  &   0.64 &   0.15 &  $-$1.23 &  \\
RAVE J074824.3-483141 & 	... & 	 +0.06$\pm$0.30 [1] & 	 +0.20$\pm$0.30 & 	6.62 & 	 +0.53$\pm$0.10 [2] &	 +0.44$\pm$0.20 [2]  &	 +0.33$\pm$0.20 [2 ] &	 +0.11$\pm$0.28 \\	 &  &  &  &  &   1.39 &   0.61 &  $-$1.16 &  \\
RAVE J100709.2-180947 & 	$r$-I & 	  $-$0.22$\pm$0.30 [1] & 	 +0.23$\pm$0.30 & 	6.74 & 	 ... &	 +0.24$\pm$0.20 [1]  &	 +0.35$\pm$0.20 [3 ] &	  $-$0.12$\pm$0.28 \\	 &  &  &  &  &  ... &   0.50 &  $-$1.05 &  \\
RAVE J100824.9-231412 & 	CEMP-$r$ & 	 +0.40$\pm$0.30 [1] & 	 +0.78$\pm$0.30 & 	7.26 & 	 ... &	 +0.36$\pm$0.20 [2]  &	 +0.55$\pm$0.20 [1 ] &	  $-$0.19$\pm$0.28 \\	 &  &  &  &  &  ... &   0.59 &  $-$0.88 &  \\
RAVE J101621.6-295952 & 	... & 	 +0.02$\pm$0.30 [1] & 	 +0.08$\pm$0.30 & 	6.39 & 	 +0.23$\pm$0.20 [1] &	  $-$0.07$\pm$0.20 [2]  &	 +0.19$\pm$0.20 [3 ] &	  $-$0.26$\pm$0.28 \\	 &  &  &  &  &   0.98 &  $-$0.01 &  $-$1.41 &  \\
RAVE J112651.4-180530 & 	... & 	 +0.25$\pm$0.30 [1] & 	 +0.26$\pm$0.30 & 	6.17 & 	  $-$0.13$\pm$0.15 [2] &	  $-$0.39$\pm$0.20 [1]  &	 ... &	 ... \\	 &  &  &  &  &   0.22 &  $-$0.73 &  ... &  \\
RAVE J113508.3-111328 & 	$r$-II & 	  $-$0.10$\pm$0.30 [1] & 	  $-$0.10$\pm$0.30 & 	7.01 & 	 +0.35$\pm$0.14 [2] &	 +0.40$\pm$0.20 [2]  &	 +0.95$\pm$0.20 [2 ] &	  $-$0.55$\pm$0.28 \\	 &  &  &  &  &   1.90 &   1.26 &   0.15 &  \\
RAVE J114444.8-112817 & 	$r$-I & 	  $-$0.10$\pm$0.30 [1] & 	  $-$0.09$\pm$0.30 & 	5.71 & 	  $-$0.01$\pm$0.10 [2] &	 +0.10$\pm$0.20 [2]  &	 +0.33$\pm$0.20 [2 ] &	  $-$0.23$\pm$0.28 \\	 &  &  &  &  &   0.23 &  $-$0.35 &  $-$1.78 &  \\
RAVE J115337.3-020037 & 	CEMP-$r$ & 	 +1.01$\pm$0.30 [1] & 	 +1.03$\pm$0.30 & 	7.03 & 	 +0.33$\pm$0.20 [1] &	 +0.54$\pm$0.20 [2]  &	 +1.11$\pm$0.20 [3 ] &	  $-$0.57$\pm$0.28 \\	 &  &  &  &  &   0.77 &   0.29 &  $-$0.80 &  \\
RAVE J115941.7-382043 & 	$r$-I & 	  $-$0.10$\pm$0.30 [1] & 	  $-$0.08$\pm$0.30 & 	7.12 & 	 +0.17$\pm$0.20 [1] &	 +0.25$\pm$0.20 [2]  &	 +0.35$\pm$0.20 [3 ] &	  $-$0.10$\pm$0.28 \\	 &  &  &  &  &   1.81 &   1.20 &  $-$0.36 &  \\
RAVE J123550.1-313111 & 	CEMP-$r$ & 	 +0.32$\pm$0.30 [1] & 	 +0.84$\pm$0.30 & 	6.68 & 	 +0.11$\pm$0.20 [1] &	 +0.06$\pm$0.20 [2]  &	 +0.57$\pm$0.20 [3 ] &	  $-$0.51$\pm$0.28 \\	 &  &  &  &  &   0.39 &  $-$0.35 &  $-$1.50 &  \\
RAVE J115941.7-382043 & 	... & 	 +0.02$\pm$0.30 [1] & 	 +0.02$\pm$0.30 & 	6.18 & 	 +0.00$\pm$0.27 [2] &	  $-$0.32$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   0.60 &  $-$0.41 &  ... &  \\
RAVE J124718.3-555047 & 	CEMP-$s$ & 	 +0.68$\pm$0.30 [1] & 	 +0.85$\pm$0.30 & 	7.28 & 	 ... &	 +1.53$\pm$0.20 [2]  &	 +0.91$\pm$0.20 [2 ] &	 +0.61$\pm$0.28 \\	 &  &  &  &  &  ... &   1.71 &  $-$0.57 &  \\
RAVE J124753.3-390802 & 	$r$-II & 	  $-$0.58$\pm$0.30 [1] & 	 +0.16$\pm$0.30 & 	6.42 & 	 ... &	 +0.36$\pm$0.20 [2]  &	 +0.77$\pm$0.20 [1 ] &	  $-$0.40$\pm$0.28 \\	 &  &  &  &  &  ... &   0.37 &  $-$0.88 &  \\
RAVE J125728.3-512522 & 	... & 	  $-$0.11$\pm$0.30 [1] & 	 +0.49$\pm$0.30 & 	6.45 & 	 +0.10$\pm$0.20 [1] &	  $-$0.16$\pm$0.20 [2]  &	 +0.16$\pm$0.20 [3 ] &	  $-$0.32$\pm$0.28 \\	 &  &  &  &  &   0.50 &  $-$0.45 &  $-$1.79 &  \\
RAVE J125807.3-450627 & 	$r$-I & 	  $-$0.79$\pm$0.30 [1] & 	  $-$0.12$\pm$0.30 & 	6.24 & 	 ... &	 +0.26$\pm$0.20 [2]  &	 +0.64$\pm$0.20 [2 ] &	  $-$0.38$\pm$0.28 \\	 &  &  &  &  &  ... &   0.37 &  $-$0.91 &  \\
RAVE J130231.2-144805 & 	$r$-I & 	 +0.05$\pm$0.30 [1] & 	 +0.05$\pm$0.30 & 	6.73 & 	 +0.35$\pm$0.20 [1] &	 +0.39$\pm$0.20 [2]  &	 +0.55$\pm$0.20 [2 ] &	  $-$0.16$\pm$0.28 \\	 &  &  &  &  &   1.47 &   0.82 &  $-$0.68 &  \\
RAVE J130404.1-240837 & 	$r$-I & 	 +0.31$\pm$0.30 [1] & 	 +0.32$\pm$0.30 & 	6.58 & 	 +0.68$\pm$0.20 [1] &	  $-$0.07$\pm$0.20 [2]  &	 +0.48$\pm$0.20 [3 ] &	  $-$0.54$\pm$0.28 \\	 &  &  &  &  &   1.38 &  $-$0.06 &  $-$1.17 &  \\
RAVE J130455.0-371249 & 	$r$-I & 	 +0.10$\pm$0.30 [1] & 	 +0.10$\pm$0.30 & 	7.64 & 	 +0.27$\pm$0.20 [0] &	 +0.39$\pm$0.20 [1]  &	 +0.45$\pm$0.20 [2 ] &	  $-$0.06$\pm$0.28 \\	 &  &  &  &  &   2.25 &   1.68 &   0.08 &  \\
RAVE J133352.8-262354 & 	... & 	 +0.19$\pm$0.30 [1] & 	 +0.60$\pm$0.30 & 	6.76 & 	 +0.15$\pm$0.10 [2] &	  $-$0.18$\pm$0.20 [2]  &	  $-$0.03$\pm$0.20 [3 ] &	  $-$0.15$\pm$0.28 \\	 &  &  &  &  &   0.75 &  $-$0.27 &  $-$1.78 &  \\
RAVE J134723.7-314409 & 	$r$-I & 	  $-$0.06$\pm$0.30 [1] & 	  $-$0.05$\pm$0.30 & 	6.39 & 	 +0.11$\pm$0.20 [1] &	 +0.52$\pm$0.20 [2]  &	 +0.66$\pm$0.20 [3 ] &	  $-$0.14$\pm$0.28 \\	 &  &  &  &  &   0.99 &   0.71 &  $-$0.81 &  \\
RAVE J135735.4-303249 & 	$r$-I & 	 +0.21$\pm$0.30 [1] & 	 +0.22$\pm$0.30 & 	6.19 & 	  $-$0.19$\pm$0.20 [1] &	  $-$0.32$\pm$0.20 [2]  &	 +0.37$\pm$0.20 [3 ] &	  $-$0.69$\pm$0.28 \\	 &  &  &  &  &   0.22 &  $-$0.60 &  $-$1.57 &  \\
RAVE J140329.0-525043 & 	$r$-I & 	 +0.00$\pm$0.30 [1] & 	 +0.01$\pm$0.30 & 	6.51 & 	 +0.20$\pm$0.20 [1] &	 +0.04$\pm$0.20 [1]  &	 +0.39$\pm$0.20 [2 ] &	  $-$0.35$\pm$0.28 \\	 &  &  &  &  &   1.14 &   0.29 &  $-$1.02 &  \\
RAVE J140335.4-333526 & 	... & 	 +0.13$\pm$0.30 [1] & 	 +0.35$\pm$0.30 & 	6.03 & 	 +0.11$\pm$0.20 [1] &	 +0.51$\pm$0.20 [1]  &	 +0.33$\pm$0.20 [1 ] &	 +0.18$\pm$0.28 \\	 &  &  &  &  &   0.23 &  $-$0.06 &  $-$1.90 &  \\
RAVE J141126.2-113746 & 	$r$-I & 	  $-$0.06$\pm$0.30 [1] & 	 +0.66$\pm$0.30 & 	6.34 & 	 +0.04$\pm$0.20 [1] &	  $-$1.32$\pm$0.20 [2]  &	 +0.57$\pm$0.20 [2 ] &	  $-$1.89$\pm$0.28 \\	 &  &  &  &  &   0.16 &  $-$1.89 &  $-$1.66 &  \\
RAVE J141253.2-355256 & 	$r$-I & 	 +0.02$\pm$0.30 [1] & 	 +0.53$\pm$0.30 & 	6.51 & 	 +0.07$\pm$0.20 [1] &	  $-$0.01$\pm$0.20 [2]  &	 +0.35$\pm$0.20 [3 ] &	  $-$0.36$\pm$0.28 \\	 &  &  &  &  &   0.49 &  $-$0.28 &  $-$1.58 &  \\
RAVE J153830.9-180424 & 	$r$-II & 	  $-$0.16$\pm$0.30 [1] & 	 +0.37$\pm$0.30 & 	6.60 & 	 +0.36$\pm$0.20 [1] &	 +0.88$\pm$0.20 [2]  &	 +1.23$\pm$0.20 [3 ] &	  $-$0.35$\pm$0.28 \\	 &  &  &  &  &   1.03 &   0.86 &  $-$0.45 &  \\
RAVE J155211.1-143037 & 	$r$-I & 	 +0.09$\pm$0.30 [1] & 	 +0.09$\pm$0.30 & 	6.92 & 	 +0.34$\pm$0.14 [2] &	 +0.53$\pm$0.20 [2]  &	 +0.66$\pm$0.20 [2 ] &	  $-$0.13$\pm$0.28 \\	 &  &  &  &  &   1.61 &   1.11 &  $-$0.42 &  \\
RAVE J155829.6-122434 & 	$r$-II & 	  $-$0.48$\pm$0.30 [1] & 	 +0.26$\pm$0.30 & 	5.87 & 	 +0.55$\pm$0.10 [2] &	 +0.33$\pm$0.20 [2]  &	 +0.80$\pm$0.20 [3 ] &	  $-$0.47$\pm$0.28 \\	 &  &  &  &  &   0.60 &  $-$0.31 &  $-$1.50 &  \\
RAVE J160245.0-152102 & 	$r$-I & 	  $-$0.06$\pm$0.30 [1] & 	  $-$0.05$\pm$0.30 & 	6.33 & 	 +0.02$\pm$0.10 [2] &	 +0.26$\pm$0.20 [2]  &	 +0.34$\pm$0.20 [3 ] &	  $-$0.08$\pm$0.28 \\	 &  &  &  &  &   0.84 &   0.39 &  $-$1.19 &  \\
RAVE J161847.0-014540 & 	$r$-I & 	 +0.10$\pm$0.30 [1] & 	 +0.47$\pm$0.30 & 	6.81 & 	 +0.35$\pm$0.20 [1] &	 +0.31$\pm$0.20 [2]  &	 +0.34$\pm$0.20 [3 ] &	  $-$0.03$\pm$0.28 \\	 &  &  &  &  &   1.13 &   0.40 &  $-$1.23 &  \\
RAVE J161943.1-022431 & 	$r$-I & 	 +0.31$\pm$0.30 [1] & 	 +0.32$\pm$0.30 & 	6.51 & 	 +0.26$\pm$0.10 [2] &	 +0.37$\pm$0.20 [2]  &	 +0.53$\pm$0.20 [3 ] &	  $-$0.16$\pm$0.28 \\	 &  &  &  &  &   0.89 &   0.31 &  $-$1.19 &  \\
RAVE J165300.5-005507 & 	$r$-I & 	  $-$0.51$\pm$0.30 [1] & 	 +0.08$\pm$0.30 & 	6.88 & 	 +0.09$\pm$0.20 [1] &	 +0.32$\pm$0.20 [2]  &	 +0.34$\pm$0.20 [3 ] &	  $-$0.02$\pm$0.28 \\	 &  &  &  &  &   1.33 &   0.87 &  $-$0.77 &  \\
2MASS J17163340-7009028 & 	$r$-I & 	  $-$0.42$\pm$0.30 [1] & 	 +0.32$\pm$0.30 & 	6.06 & 	 ... &	  $-$0.15$\pm$0.20 [2]  &	 +0.68$\pm$0.20 [3 ] &	  $-$0.83$\pm$0.28 \\	 &  &  &  &  &  ... &  $-$0.66 &  $-$1.49 &  \\
RAVE J175159.8-475131 & 	$r$-I & 	  $-$0.70$\pm$0.30 [1] & 	  $-$0.12$\pm$0.30 & 	6.11 & 	 +0.29$\pm$0.20 [1] &	  $-$0.22$\pm$0.20 [1]  &	 +0.51$\pm$0.20 [3 ] &	  $-$0.73$\pm$0.28 \\	 &  &  &  &  &   0.96 &  $-$0.24 &  $-$1.17 &  \\
RAVE J180242.3-440443 & 	CEMP-$i$ & 	 +0.48$\pm$0.30 [1] & 	 +0.84$\pm$0.30 & 	7.39 & 	 ... &	 +0.74$\pm$0.20 [2]  &	 +0.51$\pm$0.20 [3 ] &	 +0.23$\pm$0.28 \\	 &  &  &  &  &  ... &   1.04 &  $-$0.85 &  \\
RAVE J183108.2-491105 & 	... & 	  $-$0.49$\pm$0.30 [1] & 	 +0.21$\pm$0.30 & 	6.56 & 	 +0.09$\pm$0.20 [1] &	  $-$0.09$\pm$0.20 [2]  &	 +0.26$\pm$0.20 [1 ] &	  $-$0.35$\pm$0.28 \\	 &  &  &  &  &   0.88 &   0.01 &  $-$1.30 &  \\
RAVE J183623.2-642812 & 	$r$-I & 	 +0.15$\pm$0.30 [1] & 	 +0.37$\pm$0.30 & 	6.26 & 	 +0.21$\pm$0.20 [1] &	 +0.29$\pm$0.20 [1]  &	 +0.53$\pm$0.20 [2 ] &	  $-$0.24$\pm$0.28 \\	 &  &  &  &  &   0.54 &  $-$0.07 &  $-$1.49 &  \\
2MASS J19031845-5138510 & 	$r$-I & 	  $-$0.02$\pm$0.30 [1] & 	  $-$0.01$\pm$0.30 & 	6.27 & 	 ... &	 +0.41$\pm$0.20 [2]  &	 +0.68$\pm$0.20 [2 ] &	  $-$0.27$\pm$0.28 \\	 &  &  &  &  &  ... &   0.44 &  $-$0.95 &  \\
RAVE J190733.1-415832 & 	... & 	 +0.01$\pm$0.30 [1] & 	 +0.69$\pm$0.30 & 	6.68 & 	 ... &	 +1.17$\pm$0.20 [2]  &	 +0.36$\pm$0.20 [2 ] &	 +0.81$\pm$0.28 \\	 &  &  &  &  &  ... &   0.91 &  $-$1.56 &  \\
RAVE J190923.1-435357 & 	... & 	  $-$0.48$\pm$0.30 [1] & 	 +0.21$\pm$0.30 & 	6.59 & 	 ... &	 +0.05$\pm$0.20 [2]  &	  $-$0.06$\pm$0.20 [2 ] &	 +0.11$\pm$0.28 \\	 &  &  &  &  &  ... &   0.18 &  $-$1.59 &  \\
RAVE J191755.9-544015 & 	CEMP-no & 	 +0.10$\pm$0.30 [1] & 	 +0.78$\pm$0.30 & 	6.40 & 	  $-$0.07$\pm$0.10 [2] &	  $-$0.30$\pm$0.20 [2]  &	 +0.16$\pm$0.20 [3 ] &	  $-$0.46$\pm$0.28 \\	 &  &  &  &  &  $-$0.01 &  $-$0.93 &  $-$2.13 &  \\
RAVE J192325.2-583341 & 	$r$-I & 	 +0.13$\pm$0.30 [1] & 	 +0.38$\pm$0.30 & 	6.40 & 	 +0.33$\pm$0.20 [1] &	 +0.43$\pm$0.20 [2]  &	 +0.63$\pm$0.20 [2 ] &	  $-$0.21$\pm$0.28 \\	 &  &  &  &  &   0.79 &   0.20 &  $-$1.26 &  \\
RAVE J192819.9-633935 & 	$r$-I & 	 +0.08$\pm$0.30 [1] & 	 +0.51$\pm$0.30 & 	6.54 & 	  $-$0.31$\pm$0.35 [2] &	 +0.17$\pm$0.20 [2]  &	 +0.48$\pm$0.20 [3 ] &	  $-$0.31$\pm$0.28 \\	 &  &  &  &  &   0.16 &  $-$0.05 &  $-$1.40 &  \\
RAVE J193102.8-440158 & 	$r$-I & 	  $-$0.36$\pm$0.30 [1] & 	 +0.38$\pm$0.30 & 	6.53 & 	 ... &	 +0.39$\pm$0.20 [2]  &	 +0.61$\pm$0.20 [3 ] &	  $-$0.22$\pm$0.28 \\	 &  &  &  &  &  ... &   0.29 &  $-$1.15 &  \\
RAVE J194318.7-594820 & 	... & 	 +0.20$\pm$0.30 [1] & 	 +0.21$\pm$0.30 & 	6.47 & 	 +0.19$\pm$0.20 [1] &	  $-$0.12$\pm$0.20 [2]  &	 +0.25$\pm$0.20 [1 ] &	  $-$0.37$\pm$0.28 \\	 &  &  &  &  &   0.89 &  $-$0.11 &  $-$1.40 &  \\
RAVE J194319.0-405425 & 	$r$-II & 	 +0.05$\pm$0.30 [1] & 	 +0.05$\pm$0.30 & 	6.76 & 	 +0.39$\pm$0.10 [2] &	 +0.53$\pm$0.20 [2]  &	 +0.74$\pm$0.20 [3 ] &	  $-$0.21$\pm$0.28 \\	 &  &  &  &  &   1.54 &   0.99 &  $-$0.46 &  \\
RAVE J194550.6-392631 & 	$r$-II & 	  $-$0.09$\pm$0.30 [1] & 	 +0.50$\pm$0.30 & 	5.96 & 	 +0.00$\pm$0.10 [2] &	 +0.50$\pm$0.20 [2]  &	 +0.84$\pm$0.20 [3 ] &	  $-$0.34$\pm$0.28 \\	 &  &  &  &  &  $-$0.10 &  $-$0.29 &  $-$1.61 &  \\
RAVE J200034.7-342004 & 	... & 	 +0.25$\pm$0.30 [1] & 	 +0.26$\pm$0.30 & 	6.57 & 	 +0.13$\pm$0.20 [1] &	 +0.03$\pm$0.20 [1]  &	 ... &	 ... \\	 &  &  &  &  &   0.88 &   0.09 &  ... &  \\
RAVE J200057.7-254149 & 	... & 	  $-$0.16$\pm$0.30 [1] & 	 +0.42$\pm$0.30 & 	6.76 & 	 +0.37$\pm$0.20 [1] &	 +0.16$\pm$0.20 [2]  &	 +0.28$\pm$0.20 [3 ] &	  $-$0.11$\pm$0.28 \\	 &  &  &  &  &   1.15 &   0.25 &  $-$1.29 &  \\
RAVE J201007.1-515502 & 	... & 	  $-$0.41$\pm$0.30 [1] & 	 +0.33$\pm$0.30 & 	6.20 & 	  $-$1.02$\pm$0.57 [2] &	  $-$0.49$\pm$0.20 [2]  &	  $-$0.11$\pm$0.20 [2 ] &	  $-$0.38$\pm$0.28 \\	 &  &  &  &  &  $-$0.71 &  $-$0.87 &  $-$2.15 &  \\
RAVE J202029.2-270735 & 	CEMP-$r$ & 	 +0.26$\pm$0.30 [1] & 	 +0.95$\pm$0.30 & 	6.37 & 	  $-$0.25$\pm$0.20 [1] &	  $-$0.34$\pm$0.20 [2]  &	 +0.81$\pm$0.20 [1 ] &	  $-$1.15$\pm$0.28 \\	 &  &  &  &  &  $-$0.39 &  $-$1.17 &  $-$1.68 &  \\
RAVE J202432.1-151029 & 	... & 	  $-$0.12$\pm$0.30 [1] & 	 +0.09$\pm$0.30 & 	6.81 & 	 +0.21$\pm$0.20 [1] &	 +0.19$\pm$0.20 [2]  &	 +0.30$\pm$0.20 [3 ] &	  $-$0.11$\pm$0.28 \\	 &  &  &  &  &   1.37 &   0.66 &  $-$0.89 &  \\
RAVE J202434.5-423334 & 	... & 	 +0.20$\pm$0.30 [1] & 	 +0.21$\pm$0.30 & 	5.96 & 	 +0.19$\pm$0.20 [1] &	 +0.21$\pm$0.20 [1]  &	 ... &	 ... \\	 &  &  &  &  &   0.38 &  $-$0.29 &  ... &  \\
2MASS J20264253-1656467 & 	... & 	  $-$0.52$\pm$0.30 [1] & 	 +0.15$\pm$0.30 & 	6.61 & 	 +0.24$\pm$0.20 [1] &	 +0.06$\pm$0.20 [2]  &	 +0.23$\pm$0.20 [3 ] &	  $-$0.17$\pm$0.28 \\	 &  &  &  &  &   1.14 &   0.27 &  $-$1.22 &  \\
RAVE J202654.7-595013 & 	$r$-I & 	  $-$0.09$\pm$0.30 [1] & 	  $-$0.08$\pm$0.30 & 	6.30 & 	 +0.22$\pm$0.10 [2] &	 +0.27$\pm$0.20 [2]  &	 +0.33$\pm$0.20 [3 ] &	  $-$0.06$\pm$0.28 \\	 &  &  &  &  &   1.04 &   0.40 &  $-$1.20 &  \\
RAVE J203428.4-241830 & 	... & 	 +0.01$\pm$0.30 [1] & 	 +0.62$\pm$0.30 & 	6.57 & 	  $-$0.47$\pm$0.28 [2] &	  $-$0.30$\pm$0.20 [2]  &	  $-$0.03$\pm$0.20 [3 ] &	  $-$0.27$\pm$0.28 \\	 &  &  &  &  &  $-$0.08 &  $-$0.60 &  $-$1.99 &  \\
RAVE J203622.6-071420 & 	$r$-I & 	  $-$0.37$\pm$0.30 [1] & 	 +0.37$\pm$0.30 & 	6.21 & 	 ... &	 +0.23$\pm$0.20 [1]  &	 +0.43$\pm$0.20 [2 ] &	  $-$0.20$\pm$0.28 \\	 &  &  &  &  &  ... &  $-$0.18 &  $-$1.64 &  \\
RAVE J203706.4-122125 & 	CEMP-no & 	 +0.24$\pm$0.30 [1] & 	 +0.87$\pm$0.30 & 	6.69 & 	  $-$0.01$\pm$0.17 [2] &	  $-$0.02$\pm$0.20 [2]  &	 +0.07$\pm$0.20 [3 ] &	  $-$0.09$\pm$0.28 \\	 &  &  &  &  &   0.25 &  $-$0.45 &  $-$2.02 &  \\
RAVE J204355.8-563629 & 	$r$-I & 	  $-$0.11$\pm$0.30 [1] & 	  $-$0.10$\pm$0.30 & 	6.26 & 	 +0.05$\pm$0.10 [2] &	 +0.07$\pm$0.20 [2]  &	 +0.39$\pm$0.20 [2 ] &	  $-$0.32$\pm$0.28 \\	 &  &  &  &  &   0.85 &   0.18 &  $-$1.16 &  \\
RAVE J204450.7-371400 & 	... & 	 +0.22$\pm$0.30 [1] & 	 +0.57$\pm$0.30 & 	6.28 & 	 +0.53$\pm$0.20 [1] &	  $-$0.73$\pm$0.20 [1]  &	 +0.30$\pm$0.20 [3 ] &	  $-$1.03$\pm$0.28 \\	 &  &  &  &  &   0.68 &  $-$1.27 &  $-$1.90 &  \\
RAVE J204954.4-480045 & 	... & 	 +0.10$\pm$0.30 [1] & 	 +0.11$\pm$0.30 & 	6.72 & 	 +0.03$\pm$0.10 [2] &	 +0.18$\pm$0.20 [2]  &	 +0.18$\pm$0.20 [2 ] &	 +0.00$\pm$0.28 \\	 &  &  &  &  &   1.08 &   0.54 &  $-$1.12 &  \\
RAVE J205149.7-615801 & 	$r$-I & 	 +0.00$\pm$0.30 [1] & 	 +0.01$\pm$0.30 & 	6.41 & 	 +0.00$\pm$0.10 [2] &	 +0.18$\pm$0.20 [2]  &	 +0.35$\pm$0.20 [3 ] &	  $-$0.17$\pm$0.28 \\	 &  &  &  &  &   0.84 &   0.33 &  $-$1.16 &  \\
RAVE J205609.1-133118 & 	... & 	 +0.02$\pm$0.30 [1] & 	 +0.43$\pm$0.30 & 	6.53 & 	  $-$0.02$\pm$0.10 [2] &	  $-$0.03$\pm$0.20 [2]  &	 +0.21$\pm$0.20 [3 ] &	  $-$0.24$\pm$0.28 \\	 &  &  &  &  &   0.52 &  $-$0.18 &  $-$1.60 &  \\
RAVE J210634.7-495750 & 	... & 	 +0.33$\pm$0.30 [1] & 	 +0.34$\pm$0.30 & 	5.53 & 	  $-$0.27$\pm$0.10 [2] &	  $-$1.09$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &  $-$0.64 &  $-$2.15 &  ... &  \\
RAVE J210642.9-682827 & 	$r$-II & 	 +0.21$\pm$0.30 [1] & 	 +0.25$\pm$0.30 & 	5.73 & 	 +0.23$\pm$0.10 [2] &	 +0.83$\pm$0.20 [2]  &	 +0.89$\pm$0.20 [2 ] &	  $-$0.05$\pm$0.28 \\	 &  &  &  &  &   0.15 &   0.06 &  $-$1.54 &  \\
RAVE J211525.5-150331 & 	... & 	 +0.10$\pm$0.30 [1] & 	 +0.24$\pm$0.30 & 	6.59 & 	 ... &	 +1.55$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &  ... &   1.65 &  ... &  \\
RAVE J211927.1-402908 & 	... & 	  $-$0.15$\pm$0.30 [1] & 	 +0.24$\pm$0.30 & 	6.52 & 	 +0.13$\pm$0.20 [1] &	 +0.23$\pm$0.20 [2]  &	 +0.23$\pm$0.20 [2 ] &	 +0.01$\pm$0.28 \\	 &  &  &  &  &   0.85 &   0.26 &  $-$1.40 &  \\
RAVE J212921.0-620915 & 	... & 	  $-$0.09$\pm$0.30 [1] & 	 +0.49$\pm$0.30 & 	6.46 & 	 +0.14$\pm$0.10 [2] &	  $-$0.22$\pm$0.20 [2]  &	 +0.07$\pm$0.20 [3 ] &	  $-$0.28$\pm$0.28 \\	 &  &  &  &  &   0.55 &  $-$0.50 &  $-$1.87 &  \\
RAVE J215118.3-135937 & 	$r$-I & 	 +0.15$\pm$0.30 [1] & 	 +0.19$\pm$0.30 & 	6.63 & 	 +0.35$\pm$0.20 [1] &	 +0.24$\pm$0.20 [2]  &	 +0.38$\pm$0.20 [2 ] &	  $-$0.14$\pm$0.28 \\	 &  &  &  &  &   1.23 &   0.43 &  $-$1.09 &  \\
RAVE J220211.8-441702 & 	... & 	 +0.10$\pm$0.30 [1] & 	 +0.11$\pm$0.30 & 	5.66 & 	  $-$0.37$\pm$0.10 [2] &	  $-$0.81$\pm$0.20 [2]  &	 +0.20$\pm$0.20 [1 ] &	  $-$1.01$\pm$0.28 \\	 &  &  &  &  &  $-$0.38 &  $-$1.51 &  $-$2.16 &  \\
RAVE J220403.6-402919 & 	... & 	 +0.29$\pm$0.30 [1] & 	 +0.41$\pm$0.30 & 	6.27 & 	 ... &	  $-$0.37$\pm$0.20 [2]  &	  $-$0.21$\pm$0.20 [1 ] &	  $-$0.16$\pm$0.28 \\	 &  &  &  &  &  ... &  $-$0.76 &  $-$2.26 &  \\
2MASS J22122728-6810067 & 	$r$-I & 	 +0.00$\pm$0.30 [1] & 	 +0.02$\pm$0.30 & 	6.69 & 	 +0.22$\pm$0.20 [1] &	 +0.50$\pm$0.20 [2]  &	 +0.53$\pm$0.20 [3 ] &	  $-$0.03$\pm$0.28 \\	 &  &  &  &  &   1.33 &   0.92 &  $-$0.71 &  \\
RAVE J222236.0-013827 & 	CEMP-$r$ & 	 +1.16$\pm$0.30 [1] & 	 +1.17$\pm$0.30 & 	6.78 & 	  $-$0.09$\pm$0.14 [2] &	  $-$1.22$\pm$0.20 [2]  &	 +0.66$\pm$0.20 [1 ] &	  $-$1.88$\pm$0.28 \\	 &  &  &  &  &  $-$0.04 &  $-$1.86 &  $-$1.64 &  \\
RAVE J223716.2-160801 & 	... & 	  $-$0.05$\pm$0.30 [1] & 	  $-$0.05$\pm$0.30 & 	6.17 & 	 +0.30$\pm$0.10 [2] &	  $-$0.05$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   0.96 &  $-$0.08 &  ... &  \\
RAVE J224927.6-223829 & 	$r$-I & 	  $-$0.21$\pm$0.30 [1] & 	 +0.39$\pm$0.30 & 	6.79 & 	 +0.12$\pm$0.20 [1] &	 +0.14$\pm$0.20 [2]  &	 +0.31$\pm$0.20 [2 ] &	  $-$0.17$\pm$0.28 \\	 &  &  &  &  &   0.96 &   0.29 &  $-$1.20 &  \\
RAVE J225319.9-224856 & 	CEMP-$i$ & 	 +0.72$\pm$0.30 [1] & 	 +1.08$\pm$0.30 & 	7.35 & 	 ... &	 +1.10$\pm$0.20 [2]  &	 +0.84$\pm$0.20 [3 ] &	 +0.26$\pm$0.28 \\	 &  &  &  &  &  ... &   1.12 &  $-$0.80 &  \\
RAVE J225926.9-523733 & 	... & 	  $-$0.01$\pm$0.30 [1] & 	 +0.00$\pm$0.30 & 	6.23 & 	 +0.34$\pm$0.17 [2] &	 +0.38$\pm$0.20 [2]  &	 +0.29$\pm$0.20 [2 ] &	 +0.09$\pm$0.28 \\	 &  &  &  &  &   1.01 &   0.36 &  $-$1.39 &  \\
RAVE J230222.9-683323 & 	... & 	 +0.59$\pm$0.30 [1] & 	 +0.60$\pm$0.30 & 	6.77 & 	  $-$0.18$\pm$0.20 [1] &	 +0.20$\pm$0.20 [2]  &	 ... &	 ... \\	 &  &  &  &  &   0.43 &   0.12 &  ... &  \\
RAVE J231300.0-450707 & 	CEMP-$r$ & 	 +0.40$\pm$0.30 [1] & 	 +0.83$\pm$0.30 & 	6.73 & 	  $-$0.37$\pm$0.21 [2] &	  $-$0.52$\pm$0.20 [2]  &	 +0.55$\pm$0.20 [2 ] &	  $-$1.07$\pm$0.28 \\	 &  &  &  &  &  $-$0.03 &  $-$0.87 &  $-$1.46 &  \\
2MASS J23131638-7011223 & 	... & 	  $-$0.13$\pm$0.30 [1] & 	 +0.14$\pm$0.30 & 	6.38 & 	  $-$0.21$\pm$0.10 [2] &	 +0.17$\pm$0.20 [2]  &	 +0.25$\pm$0.20 [3 ] &	  $-$0.08$\pm$0.28 \\	 &  &  &  &  &   0.47 &   0.16 &  $-$1.42 &  \\
\enddata
\end{deluxetable*}
